Orthonormal Basis in Minkowski Space

Finsler space is differentiable manifold for which Minkowski space is the fiber of the tangent bundle. To understand structure of the reference frame in Finsler space, we need to understand the structure of orthonormal basis in Minkowski space. In this paper, we considered the definition of orthonormal basis in Minkowski space, the structure of metric tensor relative to orthonormal basis, procedure of orthogonalization. Linear transformation of Minkowski space mapping at least one orthonormal basis into orthonormal basis is called motion. The set of motions of Minkowski space V generates not complete group SO(V) which acts single transitive on the basis manifold. Passive transformation of Minkowski space mapping at least one orthonormal basis into orthonormal basis is called quasimotion of Minkowski space. The set of passive transformations of Minkowski space generates passive representation of not complete group SO(V) on basis manifold. Since twin representations (active and passive) of not complete group SO(V) on basis manifold are single transitive, then we may consider definition of geometric object.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов, Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин,
Элементы теории функций и функционального анализа,
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem
{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том 1, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{q-alg-9705026}
{
I.Gelfand, V.Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники. ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная $\mathfrak{F}$\Hyph алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Mappings of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010)
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008)
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология, Использование вещественных чисел в общей топологии,
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М. Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fihtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%1%1%1-rcd форма
   {$1$-\rcd форма}%
   {1-rcd form, vector spaces}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%3%A%a b-CR квазидетерминант
   {$(^a_b)$\hyph \CR квазидетерминант}%
   {a b cr-quasideterminant}%
\Index%668%A%A CRcirc- базис модуля
   {$A\CRcirc$\Hyph базис модуля}%
   {A CRcirc basis, module over algebra}%
\Index%667%A%A CRcirc- линейно ависимое множество векторов
   {$A\CRcirc$\Hyph линейно зависимое множество векторов}%
   {CRcirc linearly dependent, Astar module over algebra}%
\Index%666%A%A CRcirc- линейно независимое множество векторов
   {$A\CRcirc$\Hyph линейно независимое множество векторов}%
   {CRcirc linearly independent, Astar module over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%693%A%A линейное отображение модулей
   {$A$\Hyph линейное отображение модулей}%
   {A linear map of modules}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) mapping}%
\Index%680%A%Acr линейное отображение модулей
   {\Acr линейное отображение модулей}%
   {Acr linear map of modules}%
\Index%764%A%ACRcirc линейная комбинация
   {$A\CRcirc$\Hyph линейная комбинация}%
   {ACRcirc linear combination}%
\Index%581%A%Arc  линейно зависимые векторы
   {$A\RCstar$\Hyph  линейно зависимые векторы}%
   {linearly dependent, A vector space}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%580%A%Arc линейно независимые векторы
   {$A\RCstar$\Hyph линейно независимые векторы}%
   {linearly independent, A vector space}%
\Index%789%A%Astar антилинейное отображение алгебры с сопряжением
   {$A\star$\Hyph антилинейное отображение алгебры с сопряжением}%
   {antilinear mapping of algebra with conjugation}%
\Index%575%A%Astar векторное пространство
   {$A\star$\Hyph векторное пространство}%
   {Astar vector space}%
\Index%583%A%Astar линейное отображение векторных пространств
   {$A\star$\Hyph линейное отображение векторных пространств}%
   {Astar linear map of vector spaces}%
\Index%660%A%Astar- модуль
   {$A\star$\Hyph модуль}%
   {Astar-module}%
\Index%665%A%Astar- произведение вектора на скаляр
   {$A\star$\Hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, Astar module}%
\Index%579%A%Astar-произведение вектора на скаляр
   {$A\star$\hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, vector space}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение матриц
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%13%C%crd производная Гато отображения \Vector f D-векторного пространства \Vector V в D-векторное пространство \Vector W
   {\crd производная Гато отображения $\Vector f$ $D$\hyph векторного пространства $\Vector V$ в $D$\hyph векторное пространство $\Vector W$}%
   {Gateaux crd derivative of map, D vector space}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\Index%649%C%стандартная компонента полилинейного отображения в ассоциативную алгебру
   {стандартная компонента полилинейного отображения в ассоциативную алгебру}%
   {standard component of polylinear map, associative algebra}%
\SetIndexSpace%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%23%D%d аффинное пространство
   {$D$\Hyph аффинное пространство}%
   {d affine space}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%20%D%Drc  линейно зависимые векторные поля
   {\Drc  линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%26%D%Drc базис в векторном расслоении
   {\Drc базис в векторном расслоении}%
   {drc basis, vector bundle}%
\Index%16%D%drc базис векторного пространства r строк
   {\drc базис векторного пространства \subs строк}%
   {drc basis, r rows vector space}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%19%D%drc векторное пространство r строк
   {\drc векторное пространство \subs строк}%
   {subs rows drc vector space}%
\Index%30%D%drc вектор-функция
   {\drc вектор\hyph функция}%
   {drc vector function}%
\Index%33%D%Drc линейно независимые векторные поля
   {\Drc линейно независимые векторные поля}%
   {linearly independent vector fields}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%70%D%drc представление группы
   {\drc представление группы}%
   {drc linear representation of group}%
\Index%38%D%drc производная Гато отображения \Vector f D- векторного пространства \Vector V в D- векторное пространство \Vector W
   {\drc производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $\Vector V$ в $D$\Hyph векторное пространство $\Vector W$}%
   {Gateaux drc derivative of map, D vector space}%
\Index%779%D%Dstar антилинейное отображение кольца с сопряжением
   {$D\star$\Hyph антилинейное отображение кольца с сопряжением}%
   {antilinear mapping of ring with conjugation}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%734%D%Dstar аффинное пространство
   {$D\star$\Hyph аффинное пространство}%
   {Dstar affine space}%
\Index%659%D%Dstar- базис модуля
   {$D\star$\Hyph базис модуля}%
   {D basis, module}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%42%D%Dstar компонента координат вектора \Vector r
   {\Ds компонента координат вектора $\Vector r$}%
   {Dstar component of coordinates of vector, D vector space}%
\Index%658%D%Dstar линейно зависимые векторы Dstar модуля
   {$D\star$\Hyph линейно зависимые векторы $D\star$\Hyph модуля}%
   {Dstar linearly dependent, module}%
\Index%657%D%Dstar линейно независимые векторы Dstar модуля
   {$D\star$\Hyph линейно независимые векторы $D\star$\Hyph модуля}%
   {Dstar linearly independent, module}%
\Index%769%D%Dstar линейный гомоморфизм
   {$D\star$\Hyph линейный гомоморфизм}%
   {Dstar linear homomorphism}%
\Index%71%D%Dstar- модуль
   {$D\star$\Hyph модуль}%
   {Dstar-module}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%40%D%Dstar-векторное пространство
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%44%D%Dstar-произведение вектора на скаляр
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index%15%D%D-векторное пространство
   {$D$\hyph векторное пространство}%
   {D vector space}%
\Index%25%D%rcd базис в векторном пространстве c строк
   {\rcd базис в векторном пространстве \sups строк}%
   {rcd basis, c rows vector space}%
\Index%32%D%rcd линейная оболочка в векторном пространстве
   {\rcd линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%726%N%n алгебра над кольцом
   {$n$\Hyph алгебра над кольцом}%
   {n algebra over ring}%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%49%R%drc базис, дуальный rcd базису в векторном пространстве
   {\drc базис, дуальный \rcd базису в векторном пространстве}%
   {basis dual to basis, rcd vector space}%
\Index%4%R%j i-RC квазидетерминант
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главный минор
   {\RC главный минор}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение матриц
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%677%R%RCcirc A- базис модуля
   {$\RCcirc A$\Hyph базис модуля}%
   {RCcirc A basis, module over algebra}%
\Index%676%R%RCcirc A- линейно ависимое множество векторов
   {$\RCcirc A$\Hyph линейно зависимое множество векторов}%
   {RCcirc linearly dependent, starA module over algebra}%
\Index%675%R%RCcirc A- линейно независимое множество векторов
   {$\RCcirc A$\Hyph линейно независимое множество векторов}%
   {RCcirc linearly independent, starA module over algebra}%
\Index%600%R%RCcirc вырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph вырожденная матрица $\mathcal A(A)$\Hyph отображений}%
   {RCcirc singular matrix of A(A) mappings}%
\Index%599%R%RCcirc вырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph вырожденная матрица эндоморфизмов}%
   {RCcirc singular matrix of endomorphisms}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph невырожденная матрица $A(A)$\Hyph отображений}%
   {RCcirc nonsingular matrix of A(A) mappings}%
\Index%598%R%RCcirc невырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph невырожденная матрица эндоморфизмов}%
   {RCcirc nonsingular matrix of endomorphisms}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%765%R%RCcircA линейная комбинация
   {$\RCcirc A$\Hyph линейная комбинация}%
   {RCcircA linear combination}%
\Index%21%R%rcd  линейно зависимые векторы
   {\rcd  линейно зависимые векторы}%
   {linearly dependent, vector space}%
\Index%22%R%rcd автоморфизм векторного пространства
   {\rcd автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%759%R%rcd аффинная плоскость
   {\rcd аффинная плоскость}%
   {rcd affine plane}%
\Index%758%R%rcd аффинное преобразование
   {\rcd аффинное преобразование}%
   {rcd affine transformation}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%111%R%rcd аффинный базис
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Index%24%R%rcd базис в векторном пространстве
   {\rcd базис в векторном пространстве}%
   {rcd basis, vector space}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%29%R%rcd векторное пространство c строк
   {\rcd векторное пространство \sups строк}%
   {sups rows rcd vector space}%
\Index%31%R%rcd изоморфизм векторных пространств
   {\rcd изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%34%R%rcd линейно независимые векторы
   {\rcd линейно независимые векторы}%
   {linearly independent, vector space}%
\Index%35%R%rcd линейное отображение векторных пространств
   {\rcd линейное отображение векторных пространств}%
   {rcd linear map of vector spaces}%
\Index%37%R%rcd линейным Tstar- представление группы
   {\rcd линейным \Ts представление группы}%
   {rcd linear Tstar representation of group}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\SetIndexSpace%
\Index%77%S%Dstar- произведением rcd линейного отображения A на скаляр
   {$D\star$\Hyph произведением \rcd линейного отображения $A$ на скаляр}%
   {Dstar product of rcd linear map over scalar}%
\Index%73%S%RCstarS,RCstarT- линейное отображение векторных пространств
   {$(\RCstar S,\RCstar T)$\Hyph линейное отображение векторных пространств}%
   {rcs rct linear map of vector spaces}%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%586%S%star A- product of Astar linear map over scalar
   {$\star A$\Hyph произведением $A\star$\Hyph линейного отображения на скаляр}%
   {starA product of Astar linear map over scalar}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%683%S%star A- произведение Acr линейного отображения на скаляр
   {$\star A$\Hyph произведение \Acr линейного отображения на скаляр}%
   {starA product of Acr linear map over scalar}%
\Index%78%S%star D-векторное пространство
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%674%S%starA- произведение вектора на скаляр
   {$\star A$\Hyph произведение вектора на скаляр}%
   {starA product of vector over scalar, starA module}%
\Index%735%S%starD аффинное пространство
   {$\star D$\Hyph аффинное пространство}%
   {starD affine space}%
\Index%75%S%starD компонента координат вектора \Vector r
   {\sD компонента координат вектора $\Vector r$}%
   {starD component of coordinates of vector, D vector space}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%82%S%starT- представление Omega1 алгебры A в Omega2 алгебре M
   {\sT представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {starT representation of algebra}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%85%S%starT- преобразование
   {\sT преобразование}%
   {starT transformation}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%80%S%starT- сдвиг
   {\sT сдвиг}%
   {starT shift}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%87%T%Tstar- векторное пространство матриц
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index%88%T%Tstar- линейная комбинация векторов
   {\Ts линейная комбинация векторов}%
   {linear composition of  vectors}%
\Index%90%T%Tstar- представление Omega1 алгебры A в Omega2 алгебре M
   {\Ts представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {Tstar representation of algebra}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%92%T%Tstar- преобразование
   {\Ts преобразование}%
   {Tstar transformation}%
\Index%93%T%Tstar- преобразование расслоения
   {\Ts преобразование расслоения}%
   {Tstar transformation of bundle}%
\Index%89%T%Tstar- сдвиг
   {\Ts сдвиг}%
   {Tstar shift}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%99%А%активное starT- представление
   {активное \sT представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%569%А%активное представление группы в многообразии базисов представления
   {активное представление группы $G(f)$ в многообразии базисов представления}%
   {active representation in basis manifold}%
\Index%715%А%активное преобразование многообразия базисов башни представлений
   {активное преобразование многообразия базисов башни представлений}%
   {active transformation of basis, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов представления
   {активное преобразование многообразия базисов представления}%
   {active transformation of basis, representation}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%106%А%антигомоморфизм расслоенных групп
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of fibered groups}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%616%А%ассоциатор R алгебры
   {ассоциатор $R$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%689%Б%базис A- модуля
   {базис $A$\Hyph модуля}%
   {basis of A module}%
\Index%766%Б%базис ACRcirc модуля
   {базис $A\CRcirc$\Hyph модуля}%
   {basis of ACRcirc module}%
\Index%767%Б%базис CRcircA модуля
   {базис $\RCcirc A$\Hyph модуля}%
   {basis of CRcircA module}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%115%Б%базис векторного пространства
   {базис векторного пространства}%
   {Basis}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%117%Б%базовый вектор представления группы Ли
   {базовый вектор представления группы Ли}%
   {basis vector of representation of Lie group}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Vector{\Omega}$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор
   {бесконечно малый генератор}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\SetIndexSpace%
\Index%123%В%вектор Килинга второго рода
   {вектор Килинга второго рода}%
   {Killing vector second type}%
\Index%782%В%вектор отображения
   {вектор отображения}%
   {vector of mapping}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%727%В%векторное пространство над полем
   {векторное пространство над полем}%
   {vector space over field}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%811%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%130%В%вырожденное линейное отображение D- векторного пространства
   {вырожденное линейное отображение $D$\Hyph векторного пространства}%
   {singular linear map, D vector space}%
\Index%131%В%вырожденное линейное отображение тела
   {вырожденное линейное отображение тела}%
   {singular linear map, division ring}%
\SetIndexSpace%
\Index%132%Г%геометрический объект в векторном пространстве
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Index%133%Г%геометрический объект в координатном представлении
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Index%698%Г%геометрический объект в координатном представлении, определённом в Omega_2- алгебре
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Index%134%Г%геометрический объект в координатном представлении, определённом в rcd векторном пространстве
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Index%719%Г%геометрический объект в координатном представлении, определённом в кортеже Omega- алгебр
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Index%704%Г%геометрический объект типа
   {геометрический объект типа $H$}%
   {geometric object of type H, representation g}%
\Index%135%Г%геометрический объект типа A
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometric object of type A, vector space}%
\Index%700%Г%геометрический объект, определённый в Omega_2- алгбре
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Index%136%Г%геометрический объект, определённый в rcd векторном пространстве
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Index%722%Г%геометрический объект, определённый в кортеже Omega- алгебр
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {drc affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%799%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%156%Д%дифференциал Гато второго порядка отображения \Vector f
   {дифференциал Гато второго порядка отображения $\Vector f$}%
   {Gateaux differential of Second Order, D vector space}%
\Index%155%Д%дифференциал Гато второго порядка отображения f
   {дифференциал Гато второго порядка отображения $f$}%
   {Gateaux differential of Second Order, division ring}%
\Index%632%Д%дифференциал Гато второго порядка отображения f алгебры
   {дифференциал Гато второго порядка отображения $f$ алгебры}%
   {Gateaux differential of Second Order, algebra}%
\Index%157%Д%дифференциал Гато отображения \Vector f нормированного D- векторного пространства V в нормированное D- векторное пространство W
   {дифференциал Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux differential of map, D vector space}%
\Index%158%Д%дифференциал Гато отображения f
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, division ring}%
\Index%628%Д%дифференциал Гато отображения алгебры
   {дифференциал Гато отображения $f$ алгебры}%
   {Gateaux differential of map, algebra}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%809%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\SetIndexSpace%
\Index%576%З%закон ассоциативности для Astar- векторного пространства
   {закон ассоциативности для $A\star$\Hyph векторного пространства}%
   {associative law, Astar vector space}%
\Index%585%З%закон ассоциативности для Astar линейных отображений векторных пространств
   {закон ассоциативности для $A\star$\Hyph линейных отображений векторных пространств}%
   {associative law for Astar linear mappings of vector spaces}%
\Index%662%З%закон ассоциативности для Astar- модуля
   {закон ассоциативности для $A\star$\Hyph модуля}%
   {associative law, Astar module over algebra}%
\Index%162%З%закон ассоциативности для Drc линейных отображений векторных расслоений
   {закон ассоциативности для \Drc линейных отображений векторных расслоений}%
   {associative law for drc linear maps of vector bundles}%
\Index%163%З%закон ассоциативности для Dstar- векторного пространства
   {закон ассоциативности для $D\star$\Hyph векторного пространства}%
   {associative law, Dstar vector space}%
\Index%164%З%закон ассоциативности для Dstar- векторных полей
   {закон ассоциативности для $\mathcal D\star$\Hyph векторных полей}%
   {associative law, Dstar vector fields}%
\Index%654%З%закон ассоциативности для Dstar- модуля
   {закон ассоциативности для $D\star$\Hyph модуля}%
   {associative law, Dstar module}%
\Index%161%З%закон ассоциативности для rcd линейных отображений векторных пространств
   {закон ассоциативности для \rcd линейных отображений векторных пространств}%
   {associative law for rcd linear maps of vector spaces}%
\Index%671%З%закон ассоциативности для starA- модуля
   {закон ассоциативности для $\star A$\Hyph модуля}%
   {associative law, starA module over algebra}%
\Index%165%З%закон ассоциативности для ковариантного starT- представления
   {закон ассоциативности для ковариантного \sT представления}%
   {associative law for covariant starT representation}%
\Index%166%З%закон ассоциативности для ковариантного Tstar- представления
   {закон ассоциативности для ковариантного \Ts представления}%
   {associative law for covariant Tstar representation}%
\Index%167%З%закон ассоциативности для парных представлений
   {закон ассоциативности для парных представлений}%
   {associative law for twin representations}%
\Index%168%З%закон ассоциативности произведения расслоенных соответствий
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index%577%З%закон дистрибутивности для Astar- векторного пространства
   {закон дистрибутивности для $A\star$\Hyph векторного пространства}%
   {distributive law, Astar vector space}%
\Index%663%З%закон дистрибутивности для Astar- модуля
   {закон дистрибутивности для $A\star$\Hyph модуля}%
   {distributive law, Astar module over algebra}%
\Index%169%З%закон дистрибутивности для Dstar- векторного пространства
   {закон дистрибутивности для $D\star$\Hyph векторного пространства}%
   {distributive law, Dstar vector space}%
\Index%170%З%закон дистрибутивности для Dstar- векторных полей
   {закон дистрибутивности для $\mathcal D\star$\Hyph векторных полей}%
   {distributive law, Dstar vector fields}%
\Index%655%З%закон дистрибутивности для Dstar- модуля
   {закон дистрибутивности для $D\star$\Hyph модуля}%
   {distributive law, Dstar module}%
\Index%672%З%закон дистрибутивности для starA- модуля
   {закон дистрибутивности для $\star A$\Hyph модуля}%
   {distributive law, starA module over algebra}%
\Index%578%З%закон унитарности для Astar- векторного пространства
   {закон унитарности для $A\star$\Hyph векторного пространства}%
   {unitarity law, Astar vector space}%
\Index%664%З%закон унитарности для Astar- модуля
   {закон унитарности для $A\star$\Hyph модуля}%
   {unitarity law, Astar module over algebra}%
\Index%171%З%закон унитарности для Dstar- векторного пространства
   {закон унитарности для $D\star$\Hyph векторного пространства}%
   {unitarity law, Dstar vector space}%
\Index%172%З%закон унитарности для Dstar- векторных полей
   {закон унитарности для $\mathcal D\star$\Hyph векторных полей}%
   {unitarity law, Dstar vector fields}%
\Index%656%З%закон унитарности для Dstar- модуля
   {закон унитарности для $D\star$\Hyph модуля}%
   {unitarity law, Dstar module}%
\Index%673%З%закон унитарности для starA- модуля
   {закон унитарности для $\star A$\Hyph модуля}%
   {unitarity law, starA module over algebra}%
\SetIndexSpace%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%810%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%176%К%категория Tstar- представлений Omega1 алгебры A
   {категория \Ts представлений $\Omega$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Index%177%К%категория Tstar- представлений Omega1 алгебры из категории A
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%800%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of mappings}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%741%К%кватернионная алгебра
   {кватернионная алгебра}%
   {quaternion algebra}%
\Index%184%К%ковариантное starT- представление группы
   {ковариантное \sT представление группы}%
   {covariant starT representation of group}%
\Index%185%К%ковариантное starT- представление расслоенной группы
   {ковариантное \sT представление расслоенной группы}%
   {covariant starT representation of fibered group}%
\Index%186%К%ковариантное Tstar- представление группы
   {ковариантное \Ts представление группы}%
   {covariant Tstar representation of group}%
\Index%187%К%ковариантное Tstar- представление расслоенной группы
   {ковариантное \Ts представление расслоенной группы}%
   {covariant Tstar representation of fibered group}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%614%К%коммутатор R алгебры
   {коммутатор $R$\Hyph алгебры}%
   {commutator of algebra}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%192%К%компонента линейного отображения D- векторного пространчства
   {компонента линейного отображения $D$\Hyph векторного пространчства}%
   {component of linear map, D vector space}%
\Index%193%К%компонента линейного отображения f тела
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Index%194%К%компонента полилинейного отображения \Vector A
   {компонента полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Index%647%К%компонента полилинейного отображения ассоциативной алгебры
   {компонента полилинейного отображения ассоциативной алгебры}%
   {component of polylinear map, associative algebra}%
\Index%195%К%компонента полилинейного отображения тела
   {компонента полилинейного отображения тела}%
   {component of polylinear map, division ring}%
\Index%196%К%компонента производной Гато второго порядка отображения \Vector f(\Vector x)
   {компонента производной Гато второго порядка отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Index%633%К%компонента производной Гато второго порядка отображения f(x) алгебры
   {компонента производной Гато второго порядка отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of Second Order, algebra}%
\Index%197%К%компонента производной Гато второго порядка отображения тела
   {компонента производной Гато второго порядка отображения тела}%
   {component of Gateaux derivative of Second Order, division ring}%
\Index%199%К%компонента производной Гато отображения \Vector f(\Vector x)
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space}%
\Index%198%К%компонента производной Гато отображения f(x)
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, division ring}%
\Index%629%К%компонента производной Гато отображения f(x) алгебры
   {компонента производной Гато отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of map, algebra}%
\Index%202%К%контравариантное starT- представление группы
   {контравариантное \sT представление группы}%
   {contravariant starT representation of group}%
\Index%200%К%контравариантное starT- представление расслоенной группы
   {контравариантное \sT представление расслоенной группы}%
   {contravariant starT representation of fibered group}%
\Index%201%К%контравариантное Tstar- представление группы
   {контравариантное \Ts представление группы}%
   {contravariant Tstar representation of group}%
\Index%203%К%контравариантное Tstar- представление расслоенной группы
   {контравариантное \Ts представление расслоенной группы}%
   {contravariant Tstar representation of fibered group}%
\Index%204%К%координатная матрица вектора в rcd базисе
   {координатная матрица вектора в \rcd базисе}%
   {coordinate matrix of vector in rcd basis}%
\Index%691%К%координатная матрица вектора в базисе
   {координатная матрица вектора в базисе}%
   {coordinate matrix of vector in basis, module}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов в векторном пространстве dcr строк
   {координатная матрица множества векторов в векторном пространстве \dcr строк}%
   {coordinate matrix of set of vectors, dcr vector space}%
\Index%207%К%координатная матрица множества векторов в векторном пространстве rcd строк
   {координатная матрица множества векторов в векторном пространстве \rcd строк}%
   {coordinate matrix of set of vectors, rcd vector space}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%210%К%координатное Drc векторное расслоение
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%697%К%координатное представление в Omega_2- алгебре
   {координатное представление в $\Omega_2$\Hyph алгебре}%
   {coordinate representation, Omega_2 algebra}%
\Index%212%К%координатное представление в rcd векторном пространстве
   {координатное представление в \rcd векторном пространстве}%
   {coordinate representation, rcd vector space}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%214%К%координатный rcd изоморфизм
   {координатный \rcd изоморфизм}%
   {coordinate rcd isomorphism}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора в rcd базисе
   {координаты вектора в \rcd базисе}%
   {coordinates of vector in rcd basis}%
\Index%692%К%координаты вектора в базисе
   {координаты вектора в базисе}%
   {coordinates of vector in basis, module}%
\Index%792%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%218%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object, vector space}%
\Index%701%К%координаты геометрического объекта в Omega_2- алгбре
   {координаты геометрического объекта в $\Omega_2$\Hyph алгбре $M$}%
   {coordinates of geometric object, representation g}%
\Index%219%К%координаты геометрического объекта в rcd векторном пространстве
   {координаты геометрического объекта в \rcd векторном пространстве}%
   {coordinates of geometric object, rcd vector space}%
\Index%220%К%координаты геометрического объекта в координатном rcd векторном пространстве
   {координаты геометрического объекта в координатном \rcd векторном пространстве}%
   {coordinates of geometric object, coordinate rcd vector space}%
\Index%221%К%координаты геометрического объекта в координатном представлении
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometric object, coordinate vector space}%
\Index%721%К%координаты геометрического объекта в координатном пространстве башни представлений
   {координаты геометрического объекта в координатном пространстве башни представлений}%
   {coordinates of geometric object, coordinate tower of representations}%
\Index%699%К%координаты геометрического объекта в координатном пространстве представления
   {координаты геометрического объекта в координатном пространстве представления}%
   {coordinates of geometric object, coordinate representation}%
\Index%723%К%координаты геометрического объекта в кортеже Omega- алгебр
   {координаты геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinates of geometric object, tower of representations g}%
\Index%222%К%координаты множества векторов в dcr векторном пространстве
   {координаты множества векторов в \dcr векторном пространстве}%
   {coordinates of set of vectors, dcr vector space}%
\Index%223%К%координаты множества векторов в rcd векторном пространстве
   {координаты множества векторов в \rcd векторном пространстве}%
   {coordinates of set of vectors, rcd vector space}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%737%К%координаты точки rcd аффинного пространства относительно базиса
   {координаты точки \rcd аффинного пространства относительно базиса}%
   {coordinates in rcd affine space}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%558%К%координаты элемента представления относительно множества
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%535%К%кортеж координат элемента относительно кортежа множеств
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Index%533%К%кортеж множеств образующих башни подпредставлений
   {кортеж множеств образующих башни подпредставлений}%
   {tuple of generating sets of tower subrepresentations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%651%К%косо симметричное полилинейное отображение в ассоциативную алгебру
   {косо симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map skew symmetric, associative algebra}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%230%Л%левостороннее ковариантное представление группы
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation of group}%
\Index%231%Л%левостороннее контравариантное представление группы
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation of group}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%237%Л%левый модуль нaд кольцом
   {левый модуль нaд кольцом $D$}%
   {left module over ring}%
\Index%661%Л%левый модуль над D- алгеброй A
   {левый модуль над $D$\Hyph алгеброй $A$}%
   {left module over algebra}%
\Index%731%Л%левый сдвиг R- модуля
   {левый сдвиг $R$\Hyph модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {Tstar shift, fibered group}%
\Index%686%Л%линейная комбинация векторов A- модуля
   {линейная комбинация векторов $A$\Hyph модуля}%
   {linear combination in A module}%
\Index%98%Л%линейнное отображение тела, порождённое отображением G
   {линейное отображение тела, порождённое отображением $G$}%
   {linear map generated by map, division ring}%
\Index%688%Л%линейно зависимое множество A- модуля
   {линейно зависимое множество $A$\Hyph модуля}%
   {linear dependent vectors, module}%
\Index%687%Л%линейно независимое множество A- модуля
   {линейно независимое множество $A$\Hyph модуля}%
   {linear independent vectors, module}%
\Index%608%Л%линейное отображение  R_1 модуля в R_2 модуль
   {линейное отображение  $R_1$\Hyph модуля $A_1$ в $R_2$\Hyph модуль $A_2$}%
   {linear mapping of R_1 module into R_2 module}%
\Index%242%Л%линейное отображение D- векторных пространств над полем F
   {линейное отображение $D$\Hyph векторных пространств над полем $F$}%
   {linear map over field, vector space}%
\Index%610%Л%линейное отображение R алгебры в R алгебру
   {линейное отображение $R$\Hyph алгебры $A_1$ в $R$\Hyph алгебру $A_2$}%
   {linear mapping of R algebras}%
\Index%613%Л%линейное отображение R модуля в R модуль
   {линейное отображение $R$\Hyph модуля $A_1$ в $R$\Hyph модуль $A_2$}%
   {linear mapping of R modules}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear mapping of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%801%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {Linear Representation of Lie Group}%
\Index%740%Л%линейное преобразование rcd аффинного пространства
   {линейное преобразование \rcd аффинного пространства}%
   {linear transformation, rcd affine space}%
\Index%803%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%681%М%матрица Acr линейного отображения модуля
   {матрица \Acr линейного отображения модуля}%
   {matrix of Acr linear map}%
\Index%584%М%матрица Astar линейного отображения
   {матрица $A\star$\Hyph линейного отображения}%
   {matrix of Astar linear map}%
\Index%251%М%матрица rcd линейного отображения
   {матрица \rcd линейного отображения}%
   {matrix of rcd linear map}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear mappings}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of mappings}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения D- векторного пространства
   {матрица Якоби\Hyph Гато отображения $D$\Hyph векторного пространства}%
   {Jacobi Gateaux matrix of map, D vector space}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%257%М%многообразие базисов \rcd аффинного пространства
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Index%255%М%многообразие базисов rcd векторного пространства
   {многообразие базисов \rcd векторного пространства}%
   {basis manifold of rcd vector space}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%258%М%многообразие базисов векторного пространства
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%536%М%многообразие базисов представления
   {многообразие базисов представления}%
   {basis manifold representation F algebra}%
\Index%261%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%331%М%множество образующих подпредставления
   {множество образующих подпредставления}%
   {generating set of subrepresentation}%
\Index%332%М%множество образующих представления
   {множество образующих представления}%
   {generating set of representation}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни Tstar- представлений в башню Tstar- представлений
   {морфизм из башни \Ts представлений в башню \Ts представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\SetIndexSpace%
\Index%738%Н%начало системы координат star D аффинного пространства
   {начало системы координат $\star D$\Hyph аффинного пространства}%
   {origin of coordinate system of starD affine space}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%806%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%813%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система drc линейных уравнений
   {невырожденная система \rcd линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor, algebra}%
\Index%330%Н%невырожденный эндоморфизм представления
   {невырожденный эндоморфизм представления}%
   {regular endomorphism of representation}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%313%Н%непрерывная функция над алгебро1
   {непрерывная функция над $D$\Hyph алгебро1}%
   {continuous function, algebra}%
\Index%280%Н%непрерывная функция тела
   {непрерывная функция тела}%
   {continuous function, division ring}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%346%Н%норма на D- алгебре
   {норма на $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%793%Н%норма на кольце
   {норма на кольце}%
   {absolute value on ring}%
\Index%284%Н%норма на теле
   {норма на теле}%
   {absolute value on division ring}%
\Index%285%Н%норма отображения  тела
   {норма отображения  тела}%
   {norm of map, division ring}%
\Index%286%Н%норма отображения \Vector A нормированного D-векторного пространства
   {норма отображения $\Vector A$ нормированного $D$\hyph векторного пространства}%
   {norm of map, D vector space}%
\Index%314%Н%норма отображения в D- алгебру
   {норма отображения в $D$\Hyph алгебру}%
   {norm of map, algebra}%
\Index%343%Н%нормированная D- алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%287%Н%нормированное D- векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%794%Н%нормированное кольцо
   {нормированное кольцо}%
   {valued ring}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\SetIndexSpace%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map, division ring}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%802%О%однородное линейное представление группы Ли
   {однородное линейное представление группы Ли}%
   {homogeneous Linear Representation of Lie Group}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство группы
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%804%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%304%О%орбита Tstar- представления группы
   {орбита \Ts представления группы}%
   {orbit of Tstar  representation of group}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг rcd аффинного пространства
   {параллельный сдвиг \rcd аффинного пространства}%
   {parallel shift, rcd affine space}%
\Index%684%П%парные представления D- алгебры
   {парные представления $D$\Hyph алгебры}%
   {twin representations of D algebra}%
\Index%587%П%парные представления ассоциативной алгебры
   {парные представления ассоциативной алгебры}%
   {twin representations of associative algebra}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное starT- представление
   {пассивное \sT представление}%
   {passive starT representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%695%П%пассивное представление группы в многообразии базисов представления
   {пассивное представление группы $G(f)$ в многообразии базисов представления}%
   {passive representation in basis manifold}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%570%П%пассивное преобразование многообразия базисов представления
   {пассивное преобразование многообразия базисов представления}%
   {passive transformation of basis, representation}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%336%П%пассивное преобразование на множестве rcd базисов
   {пассивное преобразование на множестве \rcd базисов}%
   {passive transformation, vector space}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%345%П%полиалинейное косо симметричное отображение
   {полиалинейное косо симметричное отображение}%
   {polylinear map skew symmetric, division ring}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%342%П%полилинейное отображение (n)-D-векторных пространств
   {полилинейное отображение $(n)$\hyph $D$\hyph векторных пространств}%
   {polylinear map of D vector spaces}%
\Index%609%П%полилинейное отображение алгебр
   {полилинейное отображение алгебр}%
   {polylinear map of algebras}%
\Index%621%П%полилинейное отображение модулей
   {полилинейное отображение модулей}%
   {polylinear map of modules}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric, division ring}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%271%П%последовательность Коши в нормированном алгебре
   {последовательность Коши в нормированном алгебрае}%
   {Cauchy sequence, normed algebra}%
\Index%241%П%последовательность Коши в нормированном кольце
   {последовательность Коши в нормированном кольце}%
   {Cauchy sequence, normed ring}%
\Index%797%П%последовательность Коши в нормированном кольце
   {последовательность Коши в нормированном кольце}%
   {Cauchy sequence, valued ring}%
\Index%351%П%последовательность Коши в нормированном теле
   {последовательность Коши в нормированном теле}%
   {Cauchy sequence, valued division ring}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%355%П%правостороннее ковариантное представление группы
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation of group}%
\Index%356%П%правостороннее контравариантное представление группы
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation of group}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%361%П%правый модуль нaд кольцом
   {правый модуль нaд кольцом $D$}%
   {right module over ring}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%460%П%предел последовательности в нормированной алгебре
   {предел последовательности в нормированной алгебре}%
   {limit of sequence, normed algebra}%
\Index%467%П%предел последовательности в нормированном кольце
   {предел последовательности в нормированном кольце}%
   {limit of sequence, normed ring}%
\Index%795%П%предел последовательности в нормированном кольце
   {предел последовательности в нормированном кольце}%
   {limit of sequence, valued ring}%
\Index%364%П%предел последовательности в нормированном теле
   {предел последовательности в нормированном теле}%
   {limit of sequence, valued division ring}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%702%П%представитель геометрического объекта в drc векторном пространстве
   {представитель геометрического объекта в \drc векторном пространстве}%
   {representative of geometric object, drc vector space}%
\Index%703%П%представитель геометрического объекта в Omega_2- алгбре
   {представитель геометрического объекта в $\Omega_2$\Hyph алгбре}%
   {representative of geometric object, representation g}%
\Index%368%П%представитель геометрического объекта в rcd векторном пространстве
   {представитель геометрического объекта в \rcd векторном пространстве}%
   {representative of geometric object, rcd vector space}%
\Index%369%П%представитель геометрического объекта в векторном пространстве
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometric object, vector space}%
\Index%724%П%представитель геометрического объекта в кортеже Omega- алгебр
   {представитель геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {representative of geometric object, tower of representations g}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%705%П%принцип инвариантности в \drc векторном пространстве
   {принцип инвариантности в \drc векторном пространстве}%
   {invariance principle}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%385%П%принцип инвариантности в векторном пространстве
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index%384%П%принцип инвариантности в представлении универсальной алгебры
   {принцип инвариантности в представлении универсальной алгебры}%
   {invariance principle, representation g}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%390%П%произведение групп
   {произведение групп}%
   {product of groups}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%395%П%произведением объектов в категории
   {произведением объектов в категории}%
   {product of objects in category}%
\Index%396%П%производная Гато второго порядка отображения f
   {производная Гато второго порядка отображения $f$}%
   {Gateaux derivative of Second Order, division ring}%
\Index%626%П%производная Гато второго порядка отображения алгебры
   {производная Гато второго порядка отображения алгебры}%
   {Gateaux derivative of Second Order, algebra}%
\Index%397%П%производная Гато отображения f
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, division ring}%
\Index%398%П%производная Гато отображения Vector f нормированого D- векторного пространства Vector V в нормированное D- векторное пространство Vector W
   {производная Гато отображения $\Vector f$ нормированого $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux derivative of map, D vector space}%
\Index%627%П%производная Гато отображения алгебры
   {производная Гато отображения алгебры}%
   {Gateaux derivative of map, algebra}%
\Index%399%П%производная Гато порядка n отображения \Vector f
   {производная Гато порядка $n$ отображения $\Vector f$}%
   {Gateaux derivative of Order n, D vector space}%
\Index%634%П%производная Гато порядка n отображения f алгебры
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, algebra}%
\Index%400%П%производная Гато порядка n отображения f тела
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%812%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит Tstar- представления
   {пространство орбит \Ts представления}%
   {space of orbits of Ts representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%412%П%прямое произведение Tstar- представлений группы
   {прямое произведение \Ts представлений группы}%
   {direct product of Tstar representations of group}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный \Drc изоморфизм}%
   {fibered coordinate drc isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%441%С%свободное Tstar- представление группы
   {свободное \Ts представление группы}%
   {free representation of group}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль над кольцом
   {свободный модуль над кольцом}%
   {free module over ring}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%781%С%скаляр отображения
   {скаляр отображения}%
   {scalar of mapping}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато отображения f^j по переменным v^i, v^j
   {смешанная частная производная Гато отображения $f^j$ по переменным $v^i$, $v^j$}%
   {Gateaux partial derivative of Second Order, D vector space}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%456%С%стандартная F- компонента линейного отображения f
   {стандартная $F$\Hyph компонента линейного отображения $f$}%
   {standard component of linear map, division ring}%
\Index%458%С%стандартная компонента дифференциала Гато отображения f
   {стандартная компонента дифференциала Гато отображения $f$}%
   {standard component of Gateaux differential, division ring}%
\Index%459%С%стандартная компонента квадратичного отображения f над полем F
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения f тела
   {стандартная компонента полилинейного отображения $f$ тела}%
   {standard component of polylinear map, division ring}%
\Index%630%С%стандартная компонента производной Гато отображения f
   {стандартная компонента производной Гато отображения $f$}%
   {standard component of Gateaux derivative, algebra}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor, division ring}%
\Index%574%С%стандартная компонента тензора в тензорном произведении алгебр
   {стандартная компонента тензора в тензорном произведении алгебр}%
   {standard component of tensor, algebra}%
\Index%464%С%стандартное F- представление линейного отображения тела
   {стандартное $F$\Hyph представление линейного отображения тела}%
   {linear map, standard representation, division ring}%
\Index%465%С%стандартное представление дифференциала Гато отображения тела над полем F
   {стандартное представление дифференциала Гато отображения тела над полем $F$}%
   {Gateaux differential, standard representation, division ring}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%648%С%стандартное представление полилинейного отображения в ассоциативную алгебру
   {стандартное представление полилинейного отображения в ассоциативную алгебру}%
   {polylinear map, standard representation, associative algebra}%
\Index%470%С%стандартное представление полилинейного отображения тела
   {стандартное представление полилинейного отображения тела}%
   {polylinear map, standard representation, division ring}%
\Index%631%С%стандартное представление производной Гато отображения над алгеброй
   {стандартное представление производной Гато отображения над алгеброй}%
   {Gateaux derivative, standard representation, algebra}%
\Index%471%С%стандартные координаты rcd базиса
   {стандартные координаты \rcd базиса}%
   {standard coordinates of rcd basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%618%С%структурные константы алгебры над кольцом
   {структурные константы алгебры $P$ над кольцом $D$}%
   {structural constants of algebra}%
\Index%473%С%структурные константы тела D над полем F
   {структурные константы тела $D$ над полем $F$}%
   {structural constants of division ring over field}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%682%С%сумма Acr линейных отображений модуля
   {сумма \Acr линейных отображений модуля}%
   {sum of Acr linear maps, module}%
\Index%475%С%сумма rcd линейных отображений
   {сумма \rcd линейных отображений}%
   {sum of rcd linear maps, rcd vector spaces}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%323%С%суперпозиция координат эндоморфизма представления и элемента
   {суперпозиция координат эндоморфизма представления $f$ и элемента $m$}%
   {superposition of coordinates, representation}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%652%Т%тензорная степень алгебры $A$
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
\Index%763%Т%тензорная степень представления
   {тензорная степень представления}%
   {tensor power of representation}%
\Index%480%Т%тензорное произведение D- векторных пространств
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Index%481%Т%тензорное произведение Dstar векторных пространств
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Index%573%Т%тензорное произведение алгебр
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Index%482%Т%тензорное произведение колец над коммутативным кольцом
   {тензорное произведение колец над коммутативным кольцом}%
   {tensor product of rings}%
\Index%483%Т%тензорное произведение представлений
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index%762%Т%тензорное произведение представлений
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index%484%Т%тензорное произведение тел
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%487%Т%топологическое drc векторное пространство
   {топологическое \drc векторное пространство}%
   {topological drc vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\SetIndexSpace%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%493%У%уравнение Килинга
   {уравнение Килинга}%
   {Killing equation}%
\Index%494%У%уравнение Килинга второго рода
   {уравнение Килинга второго рода}%
   {Killing equation second type}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%808%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%807%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%798%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%796%Ф%фундаментальная последовательность в нормированное кольце
   {фундаментальная последовательность в нормированное кольце}%
   {fundamental sequence, valued ring}%
\Index%500%Ф%фундаментальная последовательность в нормированное теле
   {фундаментальная последовательность в нормированное теле}%
   {fundamental sequence, valued division ring}%
\Index%243%Ф%фундаментальная последовательность в нормированном алгебре
   {фундаментальная последовательность в нормированном алгебре}%
   {fundamental sequence, normed algebra}%
\Index%642%Ф%фундаментальная последовательность в нормированном кольце
   {фундаментальная последовательность в нормированном кольце}%
   {fundamental sequence, normed ring}%
\Index%502%Ф%функция \gi n D- значных переменных
   {функция $\gi n$ $D$\Hyph значных переменных}%
   {function of n D valued variables}%
\Index%501%Ф%функция D- векторного пространства V в D- векторное пространство W, дифференцируемая по Гато
   {функция $D$\Hyph векторного пространства $\Vector{V}$ в $D$\Hyph векторное пространство $\Vector W$, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, D vector space}%
\Index%625%Ф%функция алгебры, дифференцируемая по Гато
   {функция алгебры, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, algebra}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%505%Ф%функция тела, дифференцируемая по Гато
   {функция тела, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, division ring}%
\Index%506%Ф%функция, непрерывная по совокупности аргументов
   {функция, непрерывная по совокупности аргументов}%
   {function continuous with respect to set of arguments}%
\Index%805%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%620%Ц%центр алгебры
   {центр $R$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%508%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis, division ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%510%Ч%частная crd производная Гато отображения fb по переменной xa
   {частная \crd производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial crd derivative of map with respect to variable, D vector space}%
\Index%511%Ч%частная drc производная Гато отображения f^b по переменной x^a
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map with respect to variable, D vector space}%
\Index%512%Ч%частная производная Гато отображения f^j по переменной v^i
   {частная производная Гато отображения $f^j$ по переменной $v^i$}%
   {Gateaux partial derivative, D vector space}%
\Index%513%Ч%частное линейное отображение переменной v^i
   {частное линейное отображение переменной $v^i$}%
   {partial linear map of variable}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%516%Э%эффективное Tstar- представление группы
   {эффективное \Ts представление группы}%
   {effective Tstar representation of group}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%517%Э%эффективное представление Omega- алгебры A
   {эффективное представление $\Omega$\Hyph алгебры $A$}%
   {effective representation of algebra}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $R$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%522%Я%ядро линейного отображения D- векторного пространства
   {ядро линейного отображения $D$\Hyph векторного пространства}%
   {kernel of linear map, D vector space}%
\Index%523%Я%ядро линейного отображения тела
   {ядро линейного отображения тела}%
   {kernel of linear map, division ring}%
\Index%524%Я%ядро неэффективности Tstar- представления группы G
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of Tstar representation of group}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%

\CloseIndex


==> Minkowski.Example.Russian.tex <==
%auto-ignore
\input{Minkowski.Example.Eq}

\chapter{Примеры пространства Минковского}

\section{Пример пространства Минковского размерности \texorpdfstring{$2$}{2}}
\label{section: Example of Minkowski Space of Dimension 2}

Мы рассмотрим пример финслеровой метрики пространства Минковского размерности $2$
(рассматриваемая метрика является частным случаем метрики \citeBib{1004.3007}-(3))
\ShowEq{example 2 of metric of Minkowski Space}

\begin{theorem}
Финслеровая метрика, определённая равенством
\EqRef{example 2 of metric of Minkowski Space}
порождает метрику пространства Минковского
\ShowEq{example 2 of metric of Minkowski Space g}
\end{theorem}
\begin{proof}
Из равенства
\EqRef{example 2 of metric of Minkowski Space}
следует
\ShowEq{example 2 of metric of Minkowski Space 1}
\ShowEq{example 2 of metric of Minkowski Space 2}
Из равенств
\EqRef{Finsler metric},
\EqRef{example 2 of metric of Minkowski Space 1},
\EqRef{example 2 of metric of Minkowski Space 2}
следует
\ShowEq{example 2 of metric of Minkowski Space g11 1}
\ShowEq{example 2 of metric of Minkowski Space g12 1}
\ShowEq{example 2 of metric of Minkowski Space g22 1}
Равенство
\EqRef{example 2 of metric of Minkowski Space g11}
следует из равенства
\EqRef{example 2 of metric of Minkowski Space g11 1}.
Равенство
\EqRef{example 2 of metric of Minkowski Space g12}
следует из равенства
\EqRef{example 2 of metric of Minkowski Space g12 1}.
Равенство
\EqRef{example 2 of metric of Minkowski Space g22}
следует из равенства
\EqRef{example 2 of metric of Minkowski Space g22 1}.
\end{proof}

Мы начнём процедуру ортогонализации\footnote{Смотри раздел
\xRef{1107.5037}{section: Orthogonality, Minkowski space}.}
с базиса
\ShowEq{example 2, orthogonal basis 1}
Пусть
\ShowEq{example 2, orthogonal basis 2}
ортогональный базис.
Так как вектор $\Vector e'_2$ ортогонален вектору $\Vector e'_1$,
то согласно определению
\ref{definition: Minkowski orthogonality}
\ExmOrtBasis{example 2, orthogonal basis 3}
Согласно равенствам
\EqRef{example 2 of metric of Minkowski Space g11},
\EqRef{example 2 of metric of Minkowski Space g12},
\ShowEq{example 2, orthogonal basis 4}
Из равенств
\EqRef{example 2, orthogonal basis 3},
\EqRef{example 2, orthogonal basis 4}
следует
\ShowEq{example 2, orthogonal basis 5}
Из равенства
\EqRef{example 2, orthogonal basis 5}
следует, что мы можем положить
\ShowEq{example 2, orthogonal basis 6}
Согласно равенствам
\EqRef{example 2 of metric of Minkowski Space g11},
\EqRef{example 2 of metric of Minkowski Space g12},
\EqRef{example 2 of metric of Minkowski Space g22},
\EqRef{example 2, orthogonal basis 6},
\ShowEq{example 2, orthogonal basis 7}
Из равенств
\EqRef{example 2, orthogonal basis 6},
\EqRef{example 2, orthogonal basis 7}
следует
\ShowEq{example 2, orthogonal basis 8}
Следовательно, вектор $\Vector e'_1$ не ортогонален вектору $\Vector e'_2$.

Поскольку
\ShowEq{example 2, orthonormal basis 1}
то длина вектора
\ShowEq{example 2, orthonormal basis 2}
равна $1$.
Поскольку
\ShowEq{example 2, orthonormal basis 3}
то длина вектора
\ShowEq{example 2, orthonormal basis 4}
равна $1$.
Следовательно, базис $\Basis e''$ является ортонормированным базисом.
Базисы $\Basis e''$ и $\Basis e$ связаны пассивным преобразованием
\ShowEq{example 2, orthonormal basis 5}

\begin{theorem}
Компоненты метрического тензора относительно базиса $\Basis e''$
имеют вид
\ShowEq{example 2, orthonormal basis 8}
\end{theorem}
\begin{proof}
Из равенств
\EqRef{transformation of metric, Minkowski space, 1},
\EqRef{example 2, orthogonal basis 4},
\EqRef{example 2, orthonormal basis 5}
следует
\ShowEq{example 2, orthonormal basis 6 1}
Равенство
\EqRef{example 2, orthonormal basis 8 1}
следует из
\EqRef{example 2, orthonormal basis 6 1}.
Из равенств
\EqRef{transformation of metric, Minkowski space, 1},
\EqRef{example 2, orthogonal basis 7},
\EqRef{example 2, orthonormal basis 5}
следует
\ShowEq{example 2, orthonormal basis 6 2}
Равенство
\EqRef{example 2, orthonormal basis 8 2}
следует из
\EqRef{example 2, orthonormal basis 6 2}.
\end{proof}

\begin{corollary}
Относительно базиса
\EqRef{example 2, orthonormal basis 5},
матрица
\EqRef{coordinates of metric tensor, 1},
соответствующая финслеровой метрике, определённой равенством
\EqRef{example 2 of metric of Minkowski Space},
имеет вид
\ShowEq{example 2, orthonormal basis 7}
\qed
\end{corollary}

\section{Структура метрики пространства Минковского}

Теорема \ref{theorem: coordinates of metric tensor}
определяет значение $g_{kl}(\Vector e_k)$, если $k\ge l$.
Однако теорема \ref{theorem: coordinates of metric tensor}
ничего не говорит о значении $g_{kl}(\Vector e_k)$, если $k<l$.
Впечатление, что это значение произвольно, порождает серьёзную проблему.
Например, если метрика не зависит от направления,
то пространство Минковского становится евклидовым пространством и матрица
\EqRef{coordinates of metric tensor, 1}
становится диагональной матрицей; поэтому непонятно каким образом
последовательность произвольных значений сходится к $0$.

Из равенства
\EqRef{example 2, orthonormal basis 7}
следует, что значение $g_{kl}(\Vector e_k)$, $k<l$, неизвестно,
но не произвольно.
В разделе
\ref{section: Example of Minkowski Space of Dimension 2},
мы выполнили построение для финслеровой метрики, определённой равенством
\EqRef{example 2 of metric of Minkowski Space}.
Наша задача - воспроизвести эти вычисления для произвольной нормы $F$
пространства Минковского размерности $2$.

Пусть $F(\Vector v)$ - финслеровая структура
пространства Минковского размерности $2$.
Пусть $g(\Vector v)$ - метрика,
определённая равенством
\EqRef{Finsler metric}.

Мы начнём процедуру ортогонализации\footnote{Смотри раздел
\xRef{1107.5037}{section: Orthogonality, Minkowski space}.}
с базиса
\ShowEq{example 2, orthogonal basis 1}
Пусть
\ShowEq{example 2, orthogonal basis 2}
ортогональный базис.
Так как вектор $\Vector e'_2$ ортогонален вектору $\Vector e'_1$,
то согласно определению
\ref{definition: Minkowski orthogonality}
\ShowEq{example 2.2, orthogonal basis 3}
Из равенства
\EqRef{example 2.2, orthogonal basis 3}
следует, что мы можем положить
\ShowEq{example 2.2, orthogonal basis 6}
Из равенства
\EqRef{example 2.2, orthogonal basis 6}
следует
\ShowEq{example 2.2, orthogonal basis 8}

Если мы положим
\ShowEq{example 2.2, orthonormal basis 1}
то ортонормированный базис $\Basis e''_2$ имеет вид
\ShowEq{example 2.2, orthonormal basis 2}

\section{Пример \texorpdfstring{$1$}{1}
пространства Минковского размерности \texorpdfstring{$3$}{3}}

Мы рассмотрим пример финслеровой метрики пространства Минковского размерности $3$
(рассматриваемая метрика является частным случаем метрики \citeBib{1004.3007}-(3))
\ShowEq{example 3 of metric of Minkowski Space}

\begin{theorem}
\label{theorem: example 3 of metric of Minkowski Space g}
Финслеровая метрика, определённая равенством
\EqRef{example 3 of metric of Minkowski Space}
порождает метрику пространства Минковского
\ShowEq{example 3 of metric of Minkowski Space g}
\end{theorem}
\begin{proof}
Из равенства
\EqRef{example 3 of metric of Minkowski Space}
следует
\ShowEq{example 3 of metric of Minkowski Space 1}
\ShowEq{example 3 of metric of Minkowski Space 2}
\ShowEq{example 3 of metric of Minkowski Space 3}
Из равенств
\EqRef{Finsler metric},
\EqRef{example 3 of metric of Minkowski Space 1},
\EqRef{example 3 of metric of Minkowski Space 2},
\EqRef{example 3 of metric of Minkowski Space 3}
следует
\ShowEq{example 3 of metric of Minkowski Space g11 1}
\ShowEq{example 3 of metric of Minkowski Space g12 1}
\ShowEq{example 3 of metric of Minkowski Space g13 1}
\ShowEq{example 3 of metric of Minkowski Space g22 1}
\ShowEq{example 3 of metric of Minkowski Space g23 1}
\ShowEq{example 3 of metric of Minkowski Space g33 1}
Равенство
\EqRef{example 3 of metric of Minkowski Space g11}
следует из равенства
\EqRef{example 3 of metric of Minkowski Space g11 1}.
Равенство
\EqRef{example 3 of metric of Minkowski Space g12}
следует из равенства
\EqRef{example 3 of metric of Minkowski Space g12 1}.
Равенство
\EqRef{example 3 of metric of Minkowski Space g13}
следует из равенства
\EqRef{example 3 of metric of Minkowski Space g13 1}.
Равенство
\EqRef{example 3 of metric of Minkowski Space g22}
следует из равенства
\EqRef{example 3 of metric of Minkowski Space g22 1}.
Равенство
\EqRef{example 3 of metric of Minkowski Space g23}
следует из равенства
\EqRef{example 3 of metric of Minkowski Space g23 1}.
Равенство
\EqRef{example 3 of metric of Minkowski Space g33}
следует из равенства
\EqRef{example 3 of metric of Minkowski Space g33 1}.
\end{proof}

\begin{theorem}
Финслеровая метрика, определённая равенством
\EqRef{example 3 of metric of Minkowski Space},
порождает симметричное отношение ортогональности.
\end{theorem}
\begin{proof}
Мы начнём процедуру ортогонализации\footnote{Смотри раздел
\xRef{1107.5037}{section: Orthogonality, Minkowski space}.}
с базиса
\ShowEq{example 3, orthogonal basis 1}
Пусть
\ShowEq{example 3, orthogonal basis 2}
ортогональный базис.
Так как вектор $\Vector e'_2$ ортогонален вектору $\Vector e'_1$,
то согласно определению
\ref{definition: Minkowski orthogonality}
\ExmOrtBasis{example 3, orthogonal basis 3 2}
Согласно равенствам
\EqRef{example 3 of metric of Minkowski Space g11},
\EqRef{example 3 of metric of Minkowski Space g12},
\EqRef{example 3 of metric of Minkowski Space g13},
\ShowEq{example 3, orthogonal basis 4 1}
Из равенств
\EqRef{example 3, orthogonal basis 3 2},
\EqRef{example 3, orthogonal basis 4 1}
следует
\ShowEq{example 3, orthogonal basis 5 2}
Поскольку значения $e'{}^2_2$, $e'{}^3_2$ произвольны,
мы положим\footnote{Если мы положим $a=1$, $b=0$,
то легко видеть, что вектор $\Vector e_1$ ортогонален вектору $\Vector e_2$
и вектор $\Vector e_2$ ортогонален вектору $\Vector e_1$.}
\ShowEq{example 3, orthogonal basis 6 2}
Согласно теореме
\ref{theorem: example 3 of metric of Minkowski Space g}
и равенствам
\EqRef{example 3, orthogonal basis 5 2},
\EqRef{example 3, orthogonal basis 6 2},
\ShowEq{example 3, orthogonal basis 4 2}
Из равенств
\EqRef{example 3, orthogonal basis 6 2},
\EqRef{example 3, orthogonal basis 4 2}
следует
\ShowEq{example 3, orthogonal basis 8 2}
Следовательно, вектор $\Vector e'_1$ ортогонален вектору $\Vector e'_2$.

Так как вектор $\Vector e'_3$ ортогонален векторам $\Vector e'_1$, $\Vector e'_2$,
то согласно определению
\ref{definition: Minkowski orthogonality}
\ShowEq{example 3, orthogonal basis 3 3}
Из равенств
\ShowEq{example 3, orthogonal basis 3 3, 0}
следует
\ShowEq{example 3, orthogonal basis 5 3}
Из равенства
\EqRef{example 3, orthogonal basis 5 3}
следует, что мы можем положить
\ShowEq{example 3, orthogonal basis 6 3}
Согласно теореме
\ref{theorem: example 3 of metric of Minkowski Space g}
и равенству
\EqRef{example 3, orthogonal basis 6 3},
\ShowEq{example 3, orthogonal basis 4 3}
Из равенств
\EqRef{example 3, orthogonal basis 6 2},
\EqRef{example 3, orthogonal basis 6 3},
\EqRef{example 3, orthogonal basis 4 3}
следует
\ShowEq{example 3, orthogonal basis 8 3}
Следовательно, векторы $\Vector e'_1$, $\Vector e'_2$ ортогональны вектору
$\Vector e'_3$.
\end{proof}

Поскольку
\ShowEq{example 2, orthonormal basis 1}
то длина вектора
\ShowEq{example 3, orthonormal basis 2}
равна $1$.
Поскольку
\ShowEq{example 3, orthonormal basis 3 2}
то длина вектора
\ShowEq{example 3, orthonormal basis 4 2}
равна $1$.
Поскольку
\ShowEq{example 3, orthonormal basis 3 3}
то длина вектора
\ShowEq{example 3, orthonormal basis 4 3}
равна $1$.
Следовательно, базис $\Basis e''$ является ортонормированным базисом.
Базисы $\Basis e''$ и $\Basis e$ связаны пассивным преобразованием
\ShowEq{example 3, orthonormal basis 5}

\begin{theorem}
Компоненты метрического тензора относительно базиса $\Basis e''$
имеют вид
\ShowEq{example 3, orthonormal basis 8}
\end{theorem}
\begin{proof}
Из равенств
\EqRef{transformation of metric, Minkowski space, 1},
\EqRef{example 3, orthogonal basis 4 1},
\EqRef{example 3, orthonormal basis 5},
следует
\ShowEq{example 3, orthonormal basis 6 1}
Равенство
\EqRef{example 3, orthonormal basis 8 1}
следует из
\EqRef{example 3, orthonormal basis 6 1}.
Из равенств
\EqRef{transformation of metric, Minkowski space, 1},
\EqRef{example 3, orthogonal basis 4 2},
\EqRef{example 3, orthonormal basis 5},
следует
\ShowEq{example 3, orthonormal basis 6 2}
Равенство
\EqRef{example 3, orthonormal basis 8 2}
следует из
\EqRef{example 3, orthonormal basis 6 2}.
Из равенств
\EqRef{transformation of metric, Minkowski space, 1},
\EqRef{example 3, orthogonal basis 4 3},
\EqRef{example 3, orthonormal basis 5},
следует
\ShowEq{example 3, orthonormal basis 6 3}
Равенство
\EqRef{example 3, orthonormal basis 8 3}
следует из
\EqRef{example 3, orthonormal basis 6 3}.
\end{proof}

\begin{corollary}
Матрица
\EqRef{coordinates of metric tensor, 1},
соответствующая финслеровой метрике, определённой равенством
\EqRef{example 3 of metric of Minkowski Space},
является диагональной матрицей.
\qed
\end{corollary}

\section{Пример \texorpdfstring{$2$}{2}
пространства Минковского размерности \texorpdfstring{$3$}{3}}
\label{section: Example of Minkowski Space of Dimension 3}

Мы рассмотрим пример финслеровой метрики пространства Минковского размерности $3$
(рассматриваемая метрика является частным случаем метрики \citeBib{1004.3007}-(3))
\ShowEq{example 3.2 of metric of Minkowski Space}

\begin{theorem}
\label{theorem: example 3.2 of metric of Minkowski Space g}
Финслерова метрика $F^2$, определённая равенством
\EqRef{example 3.2 of metric of Minkowski Space}
порождает метрику пространства Минковского
\ShowEq{example 3.2 of metric of Minkowski Space g}
\end{theorem}
\begin{proof}
Из равенства
\EqRef{example 3.2 of metric of Minkowski Space}
следует
\ShowEq{example 3.2 of metric of Minkowski Space 1}
\ShowEq{example 3.2 of metric of Minkowski Space 2}
\ShowEq{example 3.2 of metric of Minkowski Space 3}
Из равенств
\EqRef{Finsler metric},
\EqRef{example 3.2 of metric of Minkowski Space 1},
\EqRef{example 3.2 of metric of Minkowski Space 2},
\EqRef{example 3.2 of metric of Minkowski Space 3}
следует
\ShowEq{example 3.2 of metric of Minkowski Space g11 1}
\ShowEq{example 3.2 of metric of Minkowski Space g12 1}
\ShowEq{example 3.2 of metric of Minkowski Space g13 1}
\ShowEq{example 3.2 of metric of Minkowski Space g22 1}
\ShowEq{example 3.2 of metric of Minkowski Space g23 1}
\ShowEq{example 3.2 of metric of Minkowski Space g33 1}
Равенство
\EqRef{example 3.2 of metric of Minkowski Space g11}
следует из равенства
\EqRef{example 3.2 of metric of Minkowski Space g11 1}.
Равенство
\EqRef{example 3.2 of metric of Minkowski Space g12}
следует из равенства
\EqRef{example 3.2 of metric of Minkowski Space g12 1}.
Равенство
\EqRef{example 3.2 of metric of Minkowski Space g13}
следует из равенства
\EqRef{example 3.2 of metric of Minkowski Space g13 1}.
Равенство
\EqRef{example 3.2 of metric of Minkowski Space g22}
следует из равенства
\EqRef{example 3.2 of metric of Minkowski Space g22 1}.
Равенство
\EqRef{example 3.2 of metric of Minkowski Space g23}
следует из равенства
\EqRef{example 3.2 of metric of Minkowski Space g23 1}.
Равенство
\EqRef{example 3.2 of metric of Minkowski Space g33}
следует из равенства
\EqRef{example 3.2 of metric of Minkowski Space g33 1}.
\end{proof}

\begin{theorem}
Финслерова метрика $F^2$, определённая равенством
\EqRef{example 3.2 of metric of Minkowski Space},
порождает несимметричное отношение ортогональности.
Однако существуют векторы $\Vector v$, $\Vector w$,
для которых отношение ортогональности симметрично.
\end{theorem}
\begin{proof}
Мы начнём процедуру ортогонализации\footnote{Смотри раздел
\xRef{1107.5037}{section: Orthogonality, Minkowski space}.}
с базиса
\ShowEq{example 3, orthogonal basis 1}
Пусть
\ShowEq{example 3, orthogonal basis 2}
ортогональный базис.
Так как вектор $\Vector e'_2$ ортогонален вектору $\Vector e'_1$,
то согласно определению
\ref{definition: Minkowski orthogonality}
\ExmOrtBasis{example 3.2, orthogonal basis 3 2}
Согласно равенствам
\EqRef{example 3.2 of metric of Minkowski Space g11},
\EqRef{example 3.2 of metric of Minkowski Space g12},
\EqRef{example 3.2 of metric of Minkowski Space g13},
\ShowEq{example 3.2, orthogonal basis 4 1}
Из равенств
\EqRef{example 3.2, orthogonal basis 3 2},
\EqRef{example 3.2, orthogonal basis 4 1}
следует
\ShowEq{example 3.2, orthogonal basis 5 2}
Поскольку значение $e'{}^3_2$ произвольно,
мы положим\footnote{Если мы положим $a=1$, $b=0$,
то легко видеть, что вектор $\Vector e_1$ ортогонален вектору $\Vector e_2$
и вектор $\Vector e_2$ ортогонален вектору $\Vector e_1$.}
\ShowEq{example 3.2, orthogonal basis 6 2}
Координаты вектора $\Vector e'_2$ определены с точностью до
произвольного множителя.
Поэтому, не нарушая общности, мы можем поделить
координаты вектора $\Vector e'_2$ на $a$.
При этом мы должны рассмотреть два случая.
Мы рассмотрим процедуру ортогонализации, когда $a=0$, в подразделе
\ref{subsection: Procedures of Orthogonalization, a eq 0}.
Мы увидим, что в этом случае отношение ортогонализации коммутативно.
Мы рассмотрим процедуру ортогонализации, когда $a\ne 0$, в подразделе
\ref{subsection: Procedures of Orthogonalization, a ne 0}.
Мы увидим, что в этом случае отношение ортогонализации некоммутативно.
\end{proof}

\subsection{Процедура ортогонализации базиса, (\texorpdfstring{$a=0$}{a eq 0})}
\label{subsection: Procedures of Orthogonalization, a eq 0}

Поскольку $b$ произвольно, мы можем положить $b=1$.
Следовательно, вектор $\Vector e'_2$ имеет вид
\ShowEq{example 3.2, orthogonal basis 6 2 a=0}
Согласно теореме
\ref{theorem: example 3.2 of metric of Minkowski Space g}
и равенству
\EqRef{example 3.2, orthogonal basis 6 2 a=0},
\ShowEq{example 3.2, orthogonal basis 4 2 a=0}
Из равенств
\EqRef{example 3.2, orthogonal basis 6 2},
\EqRef{example 3.2, orthogonal basis 4 2 a=0}
следует
\ShowEq{example 3.2, orthogonal basis 8 2 a=0}
Следовательно, вектор $\Vector e'_1$ ортогонален вектору $\Vector e'_2$.

Так как вектор $\Vector e'_3$ ортогонален векторам $\Vector e'_1$, $\Vector e'_2$,
то согласно определению
\ref{definition: Minkowski orthogonality}
\ShowEq{example 3.2, orthogonal basis 3 3 a=0}
Из равенств
\ShowEq{example 3.2, orthogonal basis 3 3 a=0, 0}
следует
\ShowEq{example 3.2, orthogonal basis 5 3 a=0}
Из равенства
\EqRef{example 3.2, orthogonal basis 5 3 a=0}
следует, что мы можем положить
\ShowEq{example 3.2, orthogonal basis 6 3 a=0}
Согласно теореме
\ref{theorem: example 3.2 of metric of Minkowski Space g}
и равенству
\EqRef{example 3.2, orthogonal basis 6 3 a=0},
\ShowEq{example 3.2, orthogonal basis 4 3 a=0, 1}
Из равенства
\EqRef{example 3.2, orthogonal basis 4 3 a=0, 1}
следует
\ShowEq{example 3.2, orthogonal basis 4 3 a=0}
Из равенств
\EqRef{example 3.2, orthogonal basis 6 2},
\EqRef{example 3.2, orthogonal basis 6 3 a=0},
\EqRef{example 3.2, orthogonal basis 4 3 a=0}
следует
\ShowEq{example 3.2, orthogonal basis 8 3 a=0}
Следовательно, вектор $\Vector e'_2$ ортогонален вектору
$\Vector e'_3$ и вектор $\Vector e'_1$
не ортогонален вектору $\Vector e'_3$.
%\end{proof}

Поскольку
\ShowEq{example 2, orthonormal basis 1}
то длина вектора
\ShowEq{example 3, orthonormal basis 2}
равна $1$.
Поскольку
\ShowEq{example 3.2, orthonormal basis 3 2 a=0}
то длина вектора
\ShowEq{example 3.2, orthonormal basis 4 2 a=0}
равна $1$.
Поскольку
\ShowEq{example 3.2, orthonormal basis 3 3 a=0}
то длина вектора
\ShowEq{example 3.2, orthonormal basis 4 3 a=0}
равна $1$.
Следовательно, базис $\Basis e''$ является ортонормированным базисом.
Базисы $\Basis e''$ и $\Basis e$ связаны пассивным преобразованием
\ShowEq{example 3.2, orthonormal basis 5 a=0}

\begin{theorem}
Компоненты метрического тензора относительно базиса $\Basis e''$
имеют вид
\ShowEq{example 3.2, orthonormal basis 8 a=0}
\end{theorem}
\begin{proof}
Из равенств
\EqRef{transformation of metric, Minkowski space, 1},
\EqRef{example 3.2, orthogonal basis 4 1},
\EqRef{example 3.2, orthonormal basis 5 a=0},
следует
\ShowEq{example 3.2, orthonormal basis 6 1 a=0}
Равенство
\EqRef{example 3.2, orthonormal basis 8 a=0 1}
следует из
\EqRef{example 3.2, orthonormal basis 6 1 a=0}.
Из равенств
\EqRef{transformation of metric, Minkowski space, 1},
\EqRef{example 3.2, orthogonal basis 4 2 a=0},
\EqRef{example 3.2, orthonormal basis 5 a=0},
следует
\ShowEq{example 3.2, orthonormal basis 6 2 a=0}
Равенство
\EqRef{example 3.2, orthonormal basis 8 a=0 2}
следует из
\EqRef{example 3.2, orthonormal basis 6 2 a=0}.
Из равенств
\EqRef{transformation of metric, Minkowski space, 1},
\EqRef{example 3.2, orthogonal basis 4 3 a=0},
\EqRef{example 3.2, orthonormal basis 5 a=0},
следует
\ShowEq{example 3.2, orthonormal basis 6 3 a=0}
Равенство
\EqRef{example 3.2, orthonormal basis 8 a=0 3}
следует из
\EqRef{example 3.2, orthonormal basis 6 3 a=0}.
\end{proof}

\begin{corollary}
Относительно базиса $\Basis e''$,
определённого равенством
\EqRef{example 3.2, orthonormal basis 5 a=0},
матрица
\EqRef{coordinates of metric tensor, 1},
соответствующая финслеровой метрике $F^2$, определённой равенством
\EqRef{example 3.2 of metric of Minkowski Space},
имеет вид
\ShowEq{example 3.2, orthonormal basis 7 a=0}
\qed
\end{corollary}

\subsection{Процедура ортогонализации базиса, (\texorpdfstring{$a\ne 0$}{a ne 0})}
\label{subsection: Procedures of Orthogonalization, a ne 0}

Поскольку $b$ произвольно, мы можем положить $a=1$.
Следовательно, вектор $\Vector e'_2$ имеет вид
\ShowEq{example 3.2, orthogonal basis 6 2 a=1}
Согласно теореме
\ref{theorem: example 3.2 of metric of Minkowski Space g}
и равенству
\EqRef{example 3.2, orthogonal basis 6 2 a=1},
\ShowEq{example 3.2, orthogonal basis 4 2 a=1, 1}
Из равенств
\EqRef{example 3.2, orthogonal basis 4 2 a=1, 1}
следует
\ShowEq{example 3.2, orthogonal basis 4 2 a=1}
Из равенств
\EqRef{example 3.2, orthogonal basis 6 2},
\EqRef{example 3.2, orthogonal basis 4 2 a=1}
следует
\ShowEq{example 3.2, orthogonal basis 8 2 a=1}
Полученное выражение отрицательно для любого значения $b$.
Следовательно, вектор $\Vector e'_1$ не ортогонален вектору $\Vector e'_2$.

Так как вектор $\Vector e'_3$ ортогонален векторам $\Vector e'_1$, $\Vector e'_2$,
то согласно определению
\ref{definition: Minkowski orthogonality}
\ShowEq{example 3.2, orthogonal basis 3 3 a=1}
Из равенств
\ShowEq{example 3.2, orthogonal basis 3 3 a=1, 0}
следует
\ShowEq{example 3.2, orthogonal basis 5 3 a=1}
Из равенства
\EqRef{example 3.2, orthogonal basis 5 3 a=1, 1}
следует, что мы можем положить
\ShowEq{example 3.2, orthogonal basis 6 3 a=1, 1}
Из равенств
\EqRef{example 3.2, orthogonal basis 5 3 a=1, 2},
\EqRef{example 3.2, orthogonal basis 6 3 a=1, 1}
следует
\ShowEq{example 3.2, orthogonal basis 5 3 a=1, 3}
Пусть $b\ne 0$.\footnote{Если $b=0$, то
\ShowEq{vector e2 b=0}
Из равенств
\EqRef{example 3.2, orthogonal basis 5 3 a=1, 3}
следует
\ShowEq{example 3.2, orthogonal basis 5 3 a=1 b=0, 2}
\ShowEq{example 3.2, orthogonal basis 5 3 a=1 b=0, 3}
Из равенства
\EqRef{example 3.2, orthogonal basis 5 3 a=1 b=0, 3}
следует, что $c=0$.
Из равенства
\EqRef{example 3.2, orthogonal basis 6 3 a=1, 1}
следует, что $e'{}_3^1=e'{}_3^2=0$.
Следовательно, $e'{}_3^3\ne 0$ произвольно, и не нарушая общности,
мы положим
\ShowEq{vector e3 b=0}
В подразделе
\ref{subsection: Procedures of Orthogonalization, a eq 0},
мы показали, что отношение ортогональности векторов
$\Vector e'_2$ и $\Vector e'_3$ симметрично.
Следовательно, для нас не имеет значения
порядок векторов $\Vector e'_2$, $\Vector e'_3$ в базисе.
Поскольку базис $\Basis e'$ рассмотрен в подразделе
\ref{subsection: Procedures of Orthogonalization, a eq 0},
мы не рассматриваем в этом подразделе случай
$b=0$.}
Из равенства
\EqRef{example 3.2, orthogonal basis 5 3 a=1, 3}
следует
\ShowEq{example 3.2, orthogonal basis 5 3 a=1, 4}
\ShowEq{example 3.2, orthogonal basis 5 3 a=1, 5}
Из равенства
\EqRef{example 3.2, orthogonal basis 5 3 a=1, 5}
следует
\ShowEq{example 3.2, orthogonal basis 6 3 a=1, 2}
Из равенств
\EqRef{example 3.2, orthogonal basis 6 3 a=1, 1},
\EqRef{example 3.2, orthogonal basis 6 3 a=1, 2}
следует, что $c\ne 0$ произвольно и мы можем положить $c=1$
\ShowEq{example 3.2, orthogonal basis 6 3 a=1, 3}
Пусть
\ShowEq{example 3.2, orthogonal basis 6 3 a=1, 4}
Тогда
\ShowEq{example 3.2, orthogonal basis 6 3 a=1, 5}
Векторы $\Vector e'_2$, $\Vector e'_3$ имеют похожие координаты.\footnote{Условие
\ShowEq{example 3.2, orthogonal basis 6 3 a=1, 6}
означает равенство векторов $\Vector e'_3$, $\Vector e'_3$.
Однако из равенств
\EqRef{example 3.2, orthogonal basis 6 3 a=1, 4},
\EqRef{example 3.2, orthogonal basis 6 3 a=1, 6}
следует
\ShowEq{example 3.2, orthogonal basis 6 3 a=1, 7}
Поскольку
\ShowEq{example 3.2, orthogonal basis 6 3 a=1, 8}
то равенство
\EqRef{example 3.2, orthogonal basis 6 3 a=1, 6}
невозможно.
%Из этих рассуждений следует также, что
%\ShowEq{example 3.2, orthogonal basis 6 3 a=1, 9}
}
Согласно равенствам
\EqRef{example 3.2, orthogonal basis 6 2 a=1},
\EqRef{example 3.2, orthogonal basis 4 2 a=1},
\EqRef{example 3.2, orthogonal basis 6 3 a=1, 5},
\ShowEq{example 3.2, orthogonal basis 4 3 a=1}
Так как векторы $\Vector e'_2$, $\Vector e'_3$ имеют похожие координаты,
то вектор $\Vector e'_1$ не ортогонален вектору
$\Vector e'_3$.
%Из неравенства
%\EqRef{example 3.2, orthogonal basis 6 3 a=1, 9}
%следует, что вектор $\Vector e'_3$ не ортогонален вектору
%$\Vector e'_2$.
%Из равенств
%\EqRef{example 3.2, orthogonal basis 6 2},
%\EqRef{example 3.2, orthogonal basis 6 3 a=1, 3},
%\EqRef{example 3.2, orthogonal basis 4 3 a=1}
%следует
%\ShowEq{example 3.2, orthogonal basis 8 3 a=1}
%Следовательно, вектор $\Vector e'_3$ не ортогонален векторам
%$\Vector e'_1$, $\Vector e'_2$.
%\end{proof}

Поскольку
\ShowEq{example 2, orthonormal basis 1}
то длина вектора
\ShowEq{example 3, orthonormal basis 2}
равна $1$.
Поскольку
\ShowEq{example 3.2, orthonormal basis 3 2 a=1}
то длина вектора
\ShowEq{example 3.2, orthonormal basis 4 2 a=1}
равна $1$.
Поскольку
\ShowEq{example 3.2, orthonormal basis 3 3 a=1}
то длина вектора
\ShowEq{example 3.2, orthonormal basis 4 3 a=1}
равна $1$.
Следовательно, базис $\Basis e''$ является ортонормированным базисом.

Пусть
\ShowEq{example 3.2, orthonormal basis 5 a=1 f}
Базисы $\Basis e''$ и $\Basis e$ связаны пассивным преобразованием
\ShowEq{example 3.2, orthonormal basis 5 a=1}

\begin{theorem}
\label{theorem: example 3.2, orthonormal basis, g}
Рассмотрим пространство Минковского с финслеровой метрикой, определённой равенством
\EqRef{example 3.2 of metric of Minkowski Space}.
Пусть вектор $\Vector v$ имеет координаты
\ShowEq{example 3.2, orthonormal basis, vector v}
Координаты $g(\Vector v)$ имеют вид
\ShowEq{example 3.2, orthonormal basis, g(v)}
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: example 3.2 of metric of Minkowski Space g}
и равенству
\EqRef{example 3.2, orthonormal basis, vector v},
\ShowEq{example 3.2, orthonormal basis, g(v), 1}
Равенства
\EqRef{example 3.2, orthonormal basis, g(v)}
следуют из равенств
\EqRef{example 3.2, orthonormal basis, g(v), 1}.
\end{proof}

%\ifx\texFuture\Defined
\begin{theorem}
Компоненты метрического тензора относительно базиса $\Basis e''$
имеют вид
\ShowEq{example 3.2, orthonormal basis 8 a=1 1}
\ShowEq{example 3.2, orthonormal basis 8 a=1 2}
\ShowEq{example 3.2, orthonormal basis 8 a=1 3}
\end{theorem}
\begin{proof}
Из равенств
\EqRef{transformation of metric, Minkowski space, 1},
\EqRef{example 3.2, orthogonal basis 4 1},
\EqRef{example 3.2, orthonormal basis 5 a=1},
следует
\ShowEq{example 3.2, orthonormal basis 6 1 a=1}
Равенство
\EqRef{example 3.2, orthonormal basis 8 a=1 1}
следует из
\EqRef{example 3.2, orthonormal basis 6 1 a=1}.
Из равенств
\EqRef{transformation of metric, Minkowski space, 1},
\EqRef{example 3.2, orthogonal basis 4 2 a=1},
\EqRef{example 3.2, orthonormal basis 5 a=1},
следует
\ShowEq{example 3.2, orthonormal basis 6 2 a=1, 1}
\ShowEq{example 3.2, orthonormal basis 6 2 a=1, 23}
\ShowEq{example 3.2, orthonormal basis 6 2 a=1, 33}
Равенство
\EqRef{example 3.2, orthonormal basis 8 a=1 2}
следует из
\EqRef{example 3.2, orthonormal basis 6 2 a=1, 1},
\EqRef{example 3.2, orthonormal basis 6 2 a=1, 23},
\EqRef{example 3.2, orthonormal basis 6 2 a=1, 33}.
Из равенств
\EqRef{transformation of metric, Minkowski space, 1},
\EqRef{example 3.2, orthogonal basis 4 3 a=1},
\EqRef{example 3.2, orthonormal basis 5 a=1},
следует
\ShowEq{example 3.2, orthonormal basis 6 3 a=1, 1}
\ShowEq{example 3.2, orthonormal basis 6 3 a=1, 23}
Равенство
\EqRef{example 3.2, orthonormal basis 8 a=1 3}
следует из
\EqRef{example 3.2, orthonormal basis 6 3 a=1, 1},
\EqRef{example 3.2, orthonormal basis 6 3 a=1, 23}.
\end{proof}

\begin{corollary}
Относительно базиса $\Basis e''$,
определённого равенством
\EqRef{example 3.2, orthonormal basis 5 a=1},
матрица
\EqRef{coordinates of metric tensor, 1},
соответствующая финслеровой метрике $F^2$, определённой равенством
\EqRef{example 3.2 of metric of Minkowski Space},
имеет вид
\ShowEq{example 3.2, orthonormal basis 7 a=1}
\qed
\end{corollary}
%\fi

\subsection{Пример движения в пространстве Минковского размерности \texorpdfstring{$3$}{3}}

\begin{theorem}
\label{theorem: motion Minkowski Space, 3d basis}
Рассмотрим пространство Минковского с финслеровой метрикой, определённой равенством
\EqRef{example 3.2 of metric of Minkowski Space}.

Согласно построению в подразделе
\ref{subsection: Procedures of Orthogonalization, a eq 0},
базис $\Basis e_1$, определённый равенством
\EqRef{example 3.2, orthonormal basis 5 a=0},
\ShowEq{motion Minkowski Space, 3d basis 1}
\ShowEq{motion Minkowski Space, 3d basis 1, 1}
является ортонормированным базисом.

Согласно построению в подразделе
\ref{subsection: Procedures of Orthogonalization, a ne 0},
базис $\Basis e_2$, определённый равенством
\EqRef{example 3.2, orthonormal basis 5 a=1},
\ShowEq{motion Minkowski Space, 3d basis 2}
\ShowEq{motion Minkowski Space, 3d basis 2, 1}
является ортонормированным базисом.

Рассмотрим движение $\Vector A$, отображающее базис $\Basis e_1$ в базис $\Basis e_2$
\ShowEq{motion Minkowski Space, 3d basis 1->2}
Пусть движение $\Vector A$ отображает базис $\Basis e_2$ в базис $\Basis e_3$
\ShowEq{motion Minkowski Space, 3d basis 2->3}
Базис $\Basis e_3$ не является ортонормированным базисом.
\end{theorem}
\begin{proof}
Из равенства
\EqRef{motion Minkowski Space, 3d basis 1->2}
следует
\ShowEq{motion Minkowski Space, 3d basis 1->2, 1}
Из равенства
\EqRef{motion Minkowski Space, 3d basis 1}
следует
\ShowEq{motion Minkowski Space, 3d basis 1, 2}
Из равенств
\EqRef{motion Minkowski Space, 3d basis 2},
\EqRef{motion Minkowski Space, 3d basis 1->2, 1},
\EqRef{motion Minkowski Space, 3d basis 1, 2}
следует
\ShowEq{motion Minkowski Space, 3d basis 1, 3}
Из равенств
\EqRef{motion Minkowski Space, 3d basis 2},
\EqRef{motion Minkowski Space, 3d basis 1, 3},
\EqRef{motion Minkowski Space, 3d basis 2->3}
следует
\ShowEq{motion Minkowski Space, 3d basis 3}
Пусть
\ShowEq{motion Minkowski Space, vars 1}
Тогда
\ShowEq{motion Minkowski Space, vars 2}
Поскольку последующие вычисления очень сложны, то для того,
чтобы получить ответ для конкретных значений $a$, мы написали
программу на $C\#$.
Расчёты выполнены на основании теоремы
\ref{theorem: example 3.2, orthonormal basis, g}
и равенств
\EqRef{example 3.2, orthogonal basis 6 3 a=1, 4},
\EqRef{example 3.2, orthonormal basis 5 a=1 fb},
\EqRef{example 3.2, orthonormal basis 5 a=1 fd},
\EqRef{motion Minkowski Space, vars 1}.
Утверждение теоремы следует
из расчётов, приведенных в примерах
\ref{example: motion Minkowski Space, b=1},
\ref{example: motion Minkowski Space, b=100}.
\end{proof}

\begin{example}
\label{example: motion Minkowski Space, b=1}
Пусть
\ShowEq{motion Minkowski Space, b=1}
Тогда
\ShowEq{motion Minkowski Space, b=1 d fb fd}
\ShowEq{motion Minkowski Space, b=1 e2 e3}
\ShowEq{motion Minkowski Space, b=1 g}
\ShowEq{motion Minkowski Space, b=1 g e2 e3}
\qed
\end{example}

\begin{example}
\label{example: motion Minkowski Space, b=100}
Пусть
\ShowEq{motion Minkowski Space, b=100}
Тогда
\ShowEq{motion Minkowski Space, b=100 d fb fd}
\ShowEq{motion Minkowski Space, b=100 e2 e3}
\ShowEq{motion Minkowski Space, b=100 g}
\ShowEq{motion Minkowski Space, b=100 g e2 e3}
\qed
\end{example}

\section{Пример пространства Минковского размерности \texorpdfstring{$4$}{4}}

Мы рассмотрим пример финслеровой метрики пространства Минковского размерности $4$
(рассматриваемая метрика является частным случаем метрики \citeBib{1004.3007}-(3);
мы полагаем $c=1$)
\ShowEq{example 4 of metric of Minkowski Space}
Соответствующее пространство Минковского $\Vector V$
можно представить в виде прямой суммы
\ShowEq{V=V3+R}
где $\Vector V_3$ - пространство Минковского, рассмотренное в разделе
\ref{section: Example of Minkowski Space of Dimension 3}.

Пусть
\ShowEq{Fr}
Соответственно, мы можем представить функцию $F^2$ в виде суммы
\ShowEq{F=F3+FR}
Функция $F_3^2$ является финслеровой метрикой пространства Минковского,
рассмотренного в разделе
\ref{section: Example of Minkowski Space of Dimension 3}.

\begin{theorem}
\label{theorem: F3 0 0 0}
Функция $F_3^2$ непрерывна в точке $(0,0,0)$ и может быть продолжена
по непрерывности\footnote{Значение
функции $F_3^2$ в точке $(0,0,0)$ плохо определено, так как выражение
включает отношение двух бесконечно малых.
}
\ShowEq{F3 0 0 0}
\end{theorem}
\begin{proof}
Так как
\ShowEq{square inequality}
то
\ShowEq{v ne 0}
\ShowEq{inverse square inequality}
Из неравенства
\EqRef{inverse square inequality}
и равенства
\EqRef{F3}
следует
\ShowEq{v ne 0}
\ShowEq{inverse square inequality 1}
Для заданного $\epsilon>0$ пусть
\ShowEq{delta}
Тогда из неравенства
\EqRef{inverse square inequality 1}
и требования
\ShowEq{inverse square inequality 2}
следует
\ShowEq{v ne 0}
\ShowEq{inverse square inequality 3}
Следовательно, функция $F_3^2$ непрерывна в точке $(0,0,0)$ и
\ShowEq{limit F3}
\end{proof}

\begin{theorem}
\ShowEq{F=F3+FR 2}
\end{theorem}
\begin{proof}
Равенство
\EqRef{F=F3+FR 2}
следует из равенства
\EqRef{F=F3+FR}
и теоремы
\ref{theorem: F3 0 0 0}.
\end{proof}

\begin{theorem}
\label{theorem: example 4 of metric of Minkowski Space g}
Финслерова метрика $F^2$, определённая равенством
\EqRef{example 4 of metric of Minkowski Space}
порождает метрический тензор пространства Минковского
\ShowEq{example 4 of metric of Minkowski Space g}
\end{theorem}
\begin{proof}
Равенства
\ShowEq{example 4 of metric of Minkowski Space g, ref 1}
являются следствием теоремы
\ref{theorem: example 3.2 of metric of Minkowski Space g}
и равенства
\EqRef{F=F3+FR}.
Из равенства
\EqRef{F=F3+FR}
следует
\ShowEq{F=F3+FR, 1}
Из равенств
\EqRef{Finsler metric},
\EqRef{example 4 of metric of Minkowski Space},
\EqRef{F=F3+FR, 1}
следует
\ShowEq{F=F3+FR, 2}
\end{proof}

\begin{theorem}
Если векторы
\ShowEq{e1 e2 e3 V3}
порождают ортонормированный базис пространства Минковского $\Vector V_3$,
то векторы
\ShowEq{e1 e2 e3 V}
порождают ортонормированный базис пространства Минковского $\Vector V$.
\end{theorem}
\begin{proof}
Согласно равенству
\EqRef{F=F3+FR},
если векторы
\ShowEq{a, b in V3}
ортогональны в пространстве Минковского $\Vector V_3$,
то эти векторы также ортогональны в пространстве Минковского $\Vector V$.
Следовательно, векторы $\Vector e_1$, $\Vector e_2$, $\Vector e_3$ принадлежат
ортонормированному базису пространства Минковского $\Vector V$.
Из теоремы
\ref{theorem: example 4 of metric of Minkowski Space g}
следует, что
\ShowEq{ei e0}
Следовательно, вектор $\Vector e_0$ ортогонален вектору $\Vector e_i$, $i=1$, $2$, $3$.
Согласно равенству
\EqRef{F=F3+FR 2}
\ShowEq{norm e0 -1}
\end{proof}


==> Minkowski.Space.Russian.tex <==
%auto-ignore
\input{Minkowski.Space.Eq}

\chapter{Пространство Минковского}

\section{Однородная функция}

В этой статье мы будем рассматривать векторное пространство
над полем действительных чисел $R$.

\begin{definition}
Пусть $\Vector V$ - векторное пространство.
Функция
\ShowEq{f:x in V}
называется
\AddIndex{однородная степени}{function homogeneous} $k$,
если
\DrawEq{Euler theorem}{}
\qed
\end{definition}

\begin{theorem}[Теорема Эйлера]
\label{Euler theorem}
Функция $f(\Vector x)$, однородная степени $k$,
удовлетворяет дифференциальному уравнению
\ShowEq{Euler theorem, 2}
\end{theorem}
\begin{proof}
Продифференцируем равенство
\EqRef{Euler theorem, 2}
по $a$
\ShowEq{Euler theorem, 4}
Согласно правилу дифференцирования по частям, мы имеем
\ShowEq{Euler theorem, 5}
Из равенств \EqRef{Euler theorem, 4},
\EqRef{Euler theorem, 5} следует
\ShowEq{Euler theorem, 6}
Равенство \EqRef{Euler theorem, 2}
следует из равенства \EqRef{Euler theorem, 6}
если положить $a=1$.
\end{proof}

\begin{theorem}
\label{theorem: Euler theorem, 1}
Если $f(\Vector x)$ - функция, однородная степени $k$,
то частные производные
\ShowEq{Euler theorem, 3}
являются функциями, однородными степени $k-1$.
\end{theorem}
\begin{proof}
Рассмотрим равенство\footnote{Аналогичное доказательство смотри в
\citeBib{978-0719033414}, с. 265.}
\DrawEq{Euler theorem}{22}
Продифференцируем равенство
\eqRef{Euler theorem}{22}
по $x^i$
\ShowEq{Euler theorem, 9}
Из равенства
\EqRef{Euler theorem, 9} следует
\ShowEq{Euler theorem, 10}
Следовательно, производные
\ShowEq{Euler theorem, 3}
являются однородными функциями степени $k-1$.
\end{proof}

Если отображение
\ShowEq{f:R->R}
однородно степени $0$, то
\ShowEq{f:R->R 1}
В общем случае, мы можем только утверждать, что
\ShowEq{f:V->}
Мы будем также говорить, что отображение $f$ постоянно в направлении $\Vector x$.

\section{Финслерово пространство}

Определения в этом разделе даны по аналогии
с определениями в \citeBib{1004.3007}.

\begin{definition}
\label{definition: Minkowski space, Finsler}
Векторное пространство $V$ называется
\AddIndex{пространством Минковского}{Minkowski space, Finsler},\footnote{
Я рассмотрел определение пространства Минковского
согласно определению в \citeBib{Rund Finsler geometry}, с. 28 - 32,
\citeBib{Beem Dostoglou Ehrlich}, с. 44.
Хотя этот термин вызывает некоторые ассоциации со
специальной теорией относительности,
обычно из контекста ясно о какой геометрии идёт речь.}
если в векторном пространстве $V$ определена
\AddIndex{финслерова структура}{Finsler structure}
\ShowEq{Finsler structure}
такая, что
\StartLabelItem{definition: Minkowski space, Finsler}
\begin{enumerate}
\item \AddIndex{Финслерова метрика}{Finsler metric}
$F^2$ не обязательно положительно определена\footnote{Это
требование связано с тем, что мы рассматриваем приложения в
общей теории относительности.}
\item Функция
\ShowEq{Finsler structure in Minkowski space}
однородна степени $1$
\ShowEq{homogenious degree 1, finsler}
\label{item: Finsler structure in Minkowski space}
\item Пусть $\Basis e$ - базис векторного пространства $A$.
\label{item: metric tensor}
Координаты
\AddIndex{метрического тензора}{metric tensor, Minkowski space}
\ShowEq{Finsler metric}
порождают невырожденную симметричную матрицу.
\qed
\end{enumerate}
\end{definition}

Пусть $\Vector V$, $\Vector W$ - пространства Минковского одинаковой размерности.
Пусть
\ShowEq{f:V->W}
невырожденное линейное отображение.
Мы примем за общее правило (\citeBib{Rashevsky}, с. 176),
что если
\ShowEq{FV=FW}
либо
\ShowEq{FV=-FW}
где $F_V$ - финслерова структура в пространстве Минковского $\Vector V$,
$F_W$ - финслерова структура в пространстве Минковского $\Vector W$,
то мы не будем соответствующие геометрии считать существенно различными
и будем изучать лишь одну из них.
В частности, если $F(\Vector v)<0$ для любого вектора $\Vector v$, то не
нарушая общности мы можем рассматривать финслерову структуру
\ShowEq{F=-F}
вместо финслеровой структуры $F$.

\begin{definition}
Если
\ShowEq{Fv=0}
то вектор $\Vector v$ называется
\AddIndex{изотропным}{isotropic vector}.
Если
\ShowEq{Fv<0}
то вектор $\Vector v$ называется
\AddIndex{времениподобным}{timelike vector}.
В этом случае, $F(\Vector v)$ мнимое положительное число.
Если
\ShowEq{Fv>0}
то вектор $\Vector v$ называется
\AddIndex{пространственноподобным}{spacelike vector}.
В этом случае, $F(\Vector v)$ действительное положительное число.
\qed
\end{definition}

\begin{definition}
Для произвольного вектора
\ShowEq{v F(v) ne 0}
вектор
\ShowEq{unit vector}
называется \AddIndex{единичным вектором}{unit vector}
\qed
\end{definition}

\begin{remark}
\label{remark: metric tensor depends on vector}
Согласно определению
\EqRef{Finsler metric},
метрический тензор зависит от вектора $\Vector v$.
Поэтому скалярное произведение, определённое равенством
\ShowEq{scalar product, Minkowski space}
вообще говоря, некоммутативно.
\qed
\end{remark}

Пусть $\Basis e$ - базис пространства Минковского.
Поскольку вектор $\Vector v$ имеет разложение
\ShowEq{Vector v Basis e}
относительно базиса $\Basis e$, то отображение $F$ можно также представить в виде
\ShowEq{Finsler metric 1}

\ifx\texFuture\Defined
\begin{theorem}
Финслерова структура $F$ непрерывна в точке $\Vector v=\Vector 0$.
Опираясь на непрерывность функции,
мы можем положить
\[
F(\Vector 0)=0
\]
\end{theorem}
\begin{proof}
Пусть $\Vector v_i$ - последовательность векторов, имеющая пределом вектор $\Vector 0$.
Для вектора $\Vector v_i$, положим
\ShowEq{vector ui}
\end{proof}
\fi

\begin{theorem}
Финслерова структура пространства Минковского
удовлетворяет дифференциальным уравнениям
\ShowEq{Euler theorem, Minkowski space}
\end{theorem}
\begin{proof}
Равенство \EqRef{Euler theorem, Minkowski space, 1}
следует из утверждения \eqref{item: Finsler structure in Minkowski space}
определения \ref{definition: Minkowski space, Finsler}
и теоремы \ref{Euler theorem}.
Согласно теореме \ref{Euler theorem} производная
\ShowEq{Euler theorem, Minkowski space, 4}
является однородной функцией степени $0$,
откуда следует равенство \EqRef{Euler theorem, Minkowski space, 2}.

Последовательно дифференцируя функцию $F^2$, мы получим\footnote
{см. также \citeBib{Rund Finsler geometry}, с. 24.}
\ShowEq{Euler theorem, Minkowski space, 5}
Из равенств \EqRef{Euler theorem, Minkowski space, 1},
\EqRef{Euler theorem, Minkowski space, 2},
\EqRef{Euler theorem, Minkowski space, 5}
следует
\ShowEq{Euler theorem, Minkowski space, 6}
Из равенства
\EqRef{Euler theorem, Minkowski space, 6}
следует
\ShowEq{Euler theorem, Minkowski space, 7}
Равенство \EqRef{Euler theorem, Minkowski space, 3}
следует из равенств \EqRef{Euler theorem, Minkowski space, 1},
\EqRef{Euler theorem, Minkowski space, 7}.
\end{proof}

\begin{theorem}
\ShowEq{Euler theorem, Minkowski space, 8}
\end{theorem}
\begin{proof}
Равенство
\EqRef{Euler theorem, Minkowski space, 8}
является следствием равенств
\EqRef{Finsler metric},
\EqRef{Euler theorem, Minkowski space, 3}.
\end{proof}

\begin{theorem}
Метрический тензор $g_{ij}(\Vector a)$
является однородной функцией степени $0$ и удовлетворяет уравнению
\ShowEq{metric is homogenious degree 0}
\end{theorem}
\begin{proof}
Из утверждения \eqref{item: Finsler structure in Minkowski space}
определения \ref{definition: Minkowski space, Finsler}
следует, что отображение $F^2(\Vector v)$ однородно степени $2$.
Из теоремы \ref{theorem: Euler theorem, 1}
следует, что функция
\ShowEq{dF2}
однородна степени $1$.
Из теоремы \ref{theorem: Euler theorem, 1}
и определения \EqRef{Finsler metric}
следует, что функция $g_{ij}(\Vector x)$ однородна степени $0$.
Равенство \EqRef{metric is homogenious degree 0}
следует из теоремы \ref{Euler theorem}.
\end{proof}

\begin{remark}
Как отметил Рунд в
\citeBib{Rund Finsler geometry} на с. 35,
тензор
\ShowEq{tensor C, Minkowski space}
симметричен по всем индексам. Его компоненты являются однородными
функциями степени $-1$
и удовлетворяют следующим уравнениям
\ShowEq{tensor C 1, Minkowski space}
\qed
\end{remark}

\begin{theorem}
Пусть координаты тензора $g$ определены относительно
базиса $\Basis e$. Тогда
\ShowEq{metric is homogenious degree 0, 1}
\end{theorem}
\begin{proof}
Равенство
\EqRef{metric is homogenious degree 0, 1}
является следствием равенства
\EqRef{metric is homogenious degree 0},
так как
\ShowEq{infinitesimal transformation of metric, basis 2, Minkowski space}
\end{proof}

Рассмотрим бесконечно малое преобразование
\ShowEq{infinitesimal transformation, Minkowski space}
Тогда координаты метрического тензора испытывает бесконечно малое преобразование
\ShowEq{infinitesimal transformation of metric, Minkowski space}

\begin{definition}
\label{definition: Finsler space}
Многообразие $M$ называется
\AddIndex{финслеровым пространством}{Finsler space},
если его касательное пространство являются пространством
Минковского и финслерова структура
\ShowEq{Finsler structure in Finsler space}
непрерывно зависит от точки касания $x\in M$.
\qed
\end{definition}

\begin{remark}
Следствием того, что финслерова структура в касательном пространстве непрерывно
зависит от точки касания, является возможность определения дифференциала
длины кривой на многообразии
\ShowEq{length differential, finsler}
Обычно сперва определяют финслерово пространство, а потом рассматривают
касательное к нему пространство Минковского.
На самом деле порядок определений несущественен.
В этой статье, основным объектом исследования является пространство Минковского.
\qed
\end{remark}

\section{Ортогональность}

Как отметил Рунд в \citeBib{Rund Finsler geometry}, с. 47,
существуют различные определения тригонометрических функций
в пространстве Минковского.
Нас интересует прежде всего понятие ортогональности.

\begin{definition}
\label{definition: Minkowski orthogonality}
Вектор $v_2$
\AddIndex{ортогонален}{Minkowski orthogonality}
вектору $v_1$, если
\ShowEq{Minkowski orthogonality}
\qed
\end{definition}

Как мы видим из определения
\ref{definition: Minkowski orthogonality},
отношение ортогональности некоммутативно.
Это утверждение имеет следующее следствие.
Пусть $n$ - размерность пространства Минковского $\Vector V$.
Множество векторов $\Vector v$, ортогональных вектору $\Vector a$,
удовлетворяет линейному уравнению
\ShowEq{v orthogonal a}
и, следовательно, является векторным пространством размерности $n-1$.
Множество векторов $\Vector v$, которым вектор $\Vector a$ ортогонален,
удовлетворяет уравнению
\ShowEq{a orthogonal v}
Это множество, вообще говоря, не является векторным пространством.

\begin{definition}
\label{definition: Minkowski orthogonal basis}
Множество векторов
\ShowEq{orthogonal set of vectors 1, Minkowski space}
называется ортогональным, если
\ShowEq{orthogonal set of vectors 2, Minkowski space}
Базис $\Basis e$ называется
\AddIndex{ортогональным}{orthogonal basis, Minkowski space},
если его векторы формируют ортогональное множество.
\qed
\end{definition}

\begin{definition}
\label{definition: Minkowski orthonormal basis}
Базис $\Basis e$ называется
\AddIndex{ортонормированным}{orthonormal basis, Minkowski space},
если это ортогональный базис и
его векторы имеют единичную длину.
\qed
\end{definition}

Поскольку отношение ортогональности некоммутативно,
то важен порядок векторов
при определении ортогонального базиса.
Существуют различные процедуры ортогонализации
в пространстве Минковского, например,
\citeBib{Eisenhart: Riemannian Geometry}, с. 39.
Ниже мы рассмотрим процедуру ортогонализации,
предложенную в \citeBib{Kurosh: High Algebra},
с. 213 - 214.

\begin{theorem}
Пусть
\ShowEq{orthogonal set of vectors 1, Minkowski space}
- ортогональное множество не изотропных векторов. Тогда векторы
\ShowEq{orthogonal set of vectors 1, Minkowski space}
линейно независимы.
\end{theorem}
\begin{proof}
Рассмотрим равенство
\ShowEq{orthogonal set of vectors 3, Minkowski space}

Из равенства \EqRef{orthogonal set of vectors 3, Minkowski space}
следует
\ShowEq{orthogonal set of vectors 4, Minkowski space}
Поскольку вектор $\Vector e_1$ не изотропен, то
\ShowEq{orthogonal set of vectors 4 e1, Minkowski space}
Из условий
\EqRef{orthogonal set of vectors 2, Minkowski space},
\EqRef{orthogonal set of vectors 4 e1, Minkowski space}
и равенства
\EqRef{orthogonal set of vectors 4, Minkowski space}
следует $a_1=0$.

Если мы доказали, что $a^1=...=a^{m-1}=0$, то равенство
\EqRef{orthogonal set of vectors 3, Minkowski space}
примет вид
\ShowEq{orthogonal set of vectors 3 m, Minkowski space}
Из равенства \EqRef{orthogonal set of vectors 3 m, Minkowski space}
следует
\ShowEq{orthogonal set of vectors 4 m, Minkowski space}
Поскольку вектор $\Vector e_m$ не изотропен, то
\ShowEq{orthogonal set of vectors 4 em, Minkowski space}
Из условий
\EqRef{orthogonal set of vectors 2, Minkowski space},
\EqRef{orthogonal set of vectors 4 em, Minkowski space}
и равенства
\EqRef{orthogonal set of vectors 4 m, Minkowski space}
следует $a_m=0$.
\end{proof}

\begin{theorem}
\label{theorem: orthonormal basis in Minkowski space, positively defined Finsler metric}
В пространстве Минковского
с положительно определённой финслеровой метрикой существует ортонормированный базис.
\end{theorem}
\begin{proof}
Пусть $n$ - размерность пространства Минковского.
Пусть $\Basis e'$ - базис в пространстве Минковского.

Мы положим
\ShowEq{orthogonal basis 1, Minkowski space}

Допустим мы построили множество векторов
\ShowEq{set e1 em, Minkowski space}
Дополнительно предположим, что для всякого
\ShowEq{orthogonal basis 2, Minkowski space}
вектор $\Vector e_i$ является линейной комбинацией векторов
\ShowEq{orthogonal basis 3, Minkowski space}
Это предположение будет выполнено и для вектора $\Vector e_{m+1}$,
если мы этот вектор представим в виде
\ShowEq{orthogonal basis 4, Minkowski space}
так как $\Basis e'$ - базис, и вектор $\Vector e'_{m+1}$
не входит в разложение векторов
\ShowEq{set e1 em, Minkowski space}
Для выбора вектора $\Vector e_{m+1}$
мы потребуем, чтобы вектор $\Vector e_{m+1}$
был ортогонален векторам
\ShowEq{set e1 em, Minkowski space}
\ShowEq{choose em+1, Minkowski space}
Система линейных уравнений
\EqRef{choose em+1, Minkowski space}
имеет вид
\ShowEq{choose em 1, Minkowski space}
Следовательно, решение системы линейных уравнений
\EqRef{choose em+1, Minkowski space}
имеет вид
\ShowEq{choose em 2, Minkowski space}

Продолжая этот процесс, мы получим ортогональный базис $\Basis e$.
Мы можем нормировать векторы базиса $\Basis e$
согласно правилу
\ShowEq{orthogonal basis 5, Minkowski space}
\end{proof}

Рассмотрим пространство Минковского $\Vector V$ размерности $n$.
Пусть финслерова метрика $F^2$
пространства Минковского $\Vector V$ не является положительно опредённой.
Множество пространственноподобных векторов не является векторным пространством,
однако это множество содержит максимальное множество линейно независимых векторов
\ShowEq{spacelike independent vectors}
такое, что любая линейная комбинация этих векторов
является пространственноподобным вектором.
Множество $\Basis e'_+$ является базисом векторного пространства $\Vector V_+$.
Множество времениподобных векторов не является векторным пространством,
однако это множество содержит максимальное множество линейно независимых векторов
\ShowEq{timelike independent vectors}
такое, что любая линейная комбинация этих векторов
является времениподобным вектором.
Множество $\Basis e'_-$ является базисом векторного пространства $\Vector V_-$.
Выбор множеств $\Basis e'_+$, $\Basis e'_-$, а также
векторных пространств $\Vector V_+$,  $\Vector V_-$
неоднозначен.

\begin{theorem}
\label{theorem: There exists orthonormal basis +}
В пространстве Минковского $\Vector V_+$ с финслеровой структурой $F$
существует ортонормированный базис $\Basis e_+$.
Множество векторов, ортогональных векторам базиса $\Basis e_+$,
является векторным пространством $\Vector V_+^{\perp}$ размерности $n-p$.
\end{theorem}
\begin{proof}
Существование ортонормированного базиса $\Basis e_+$
в пространстве Минковского $\Vector V_+$ следует из теоремы
\ref{theorem: orthonormal basis in Minkowski space, positively defined Finsler metric}.
Вектор $\Vector v$, ортогональный векторам базиса $\Basis e_+$,
удовлетворяет системе линейных уравнений
\ShowEq{vector orthogonal to basis}
Следовательно, множество векторов $\Vector v$
порождает векторное пространство.
\end{proof}

\begin{theorem}
\label{theorem: exists orthonormal basis in Minkowski space}
В пространстве Минковского $\Vector V$,
где финслерова метрика $F^2$ не является положительно определённой,
существует ортонормированный базис $\Basis e$,
если выполнено одно из следующих условий
\StartLabelItem{theorem: exists orthonormal basis in Minkowski space}
\begin{enumerate}
%\item
%\label{item: V+perp}
%Векторное пространство $\Vector V_+^{\perp}$ имеет размерность $-1$
\item
\label{item: F V- V+}
Финслеровая метрика $F^2$ пространства Минковского $\Vector V$
имеет вид
\ShowEq{F V- V+}
где $F^2_+$, $F^2_-$ - положительно определённые финслеровы метрики.
Множество переменных
\ShowEq{v+ v-}
разбивает множество координат
\ShowEq{v}
вектора $\Vector v$
на два непересекающихся множества.
\item
\label{item: V+perp}
Существует векторное пространство $\Vector V_+$ такое,
что векторное пространство $\Vector V_+^{\perp}$
не содержит изотропных векторов\footnote{Хотя отображение
$F$ не является линейным, мы формально можем определить множество
$\ker F$ как множество изотропных векторов.
Тогда условие
\RefItem{V+perp}
можно сформулировать как следующее условие.
Существует векторное пространство $\Vector V_+$ такое, что
\[
\Vector V_+^{\perp}\cap\ker F=\emptyset
\]
}
\item
\label{item: V- V+perp}
Существуют векторные пространства $\Vector V_+$, $\Vector V_-$ такие,
что верно следующее равенство
\ShowEq{V- V+perp}
\end{enumerate}
\end{theorem}
\begin{proof}
%Размерность векторного пространства $\Vector V_-$ не может быть меньше $1$;
%в противном случае
%\ShowEq{V=V+}
%Следовательно, условие
%\RefItem{V+perp}
%является частным случаем условия
%\RefItem{V- V+perp}.
%
Если выполнено условие
\RefItem{F V- V+},
то естественно положить, что $p+q=n$;
в противном случае, существует изотропная плоскость.\footnote{Например,
если переменная $v^1$ не принадлежит множеству
\ShowEq{v+ v-}
то любой вектор вида
\ShowEq{v+ v- 1}
является изотропным вектором.
Это противоречит требованию
\RefItem{metric tensor}
невырожденности финслеровой метрики.

Однако вырожденность финслеровой метрики необязательно следует
из существования изотропной плоскости.
В псевдоевклидовом
пространстве с метрикой
\ShowEq{+-+-}
векторы
\ShowEq{+-+- 1}
являются изотропными векторами.
Вектор
\ShowEq{+-+- 2}
также является изотропным вектором.
Однако векторы
\ShowEq{+-+- +}
порождают векторное пространство $\Vector V_+$,
а векторы
\ShowEq{+-+- -}
порождают векторное пространство $\Vector V_-$.
}
Полагая
\ShowEq{F V- V+ 1}
мы видим, что векторное пространство $\Vector V_+$ имеет размерность $p$.
Полагая
\ShowEq{F V- V+ 2}
мы видим, что векторное пространство $\Vector V_-$ имеет размерность $q$.
Согласно теореме
\ref{theorem: There exists orthonormal basis +},
в пространстве Минковского $\Vector V_+$ с финслеровой структурой $F$
существует ортонормированный базис $\Basis e_+$
и размерность векторного пространства $\Vector V_+^{\perp}$
равна $n-p=q$.
Следовательно, условие
\RefItem{F V- V+}
является частным случаем условия
\RefItem{V- V+perp}.

Пространственноподобный вектор не может быть вектором
векторного пространства $\Vector V_+^{\perp}$.
В противном случае, множество $\Basis e_+$
не является максимальным множеством линейно независимых
пространственноподобный векторов.
Если условие
\RefItem{V+perp}
верно, то векторное пространство $\Vector V_+^{\perp}$
содержит только времениподобные векторы.
Следовательно, условие
\RefItem{V+perp}
эквивалентно условию
\RefItem{V- V+perp}.

Рассмотрим условие
\RefItem{V- V+perp}.
Пусть $\Basis e_+$ - ортонормированный базис пространства Минковского $\Vector V_+$.
Пусть $\Basis e_-$ - ортонормированный базис пространства Минковского $\Vector V_-$.
Согласно условие
\RefItem{V- V+perp},
каждый вектор базиса $\Basis e_-$ ортогонален всем векторам
базиса $\Basis e_+$.
Согласно определению
\ref{definition: Minkowski orthogonal basis},
базис
\ShowEq{F V- V+ 3}
является ортогональным базисом.
Поскольку каждый вектор базиса $\Basis e$ является единичным вектором,
то согласно определению
\ref{definition: Minkowski orthonormal basis},
базис
$\Basis e$
является ортонормированным базисом.
\end{proof}

\begin{theorem}
\label{theorem: coordinates of metric tensor}
Пусть $\Basis e$ - ортонормированный базис пространства Минковского.
Если мы запишем координаты метрического тензора
\ShowEq{coordinates of metric tensor}
относительно базиса $\Basis e$ в виде матрицы
\ShowEq{coordinates of metric tensor, 1}
то матрица
\EqRef{coordinates of metric tensor, 1}
является треугольной матрицей, диагональные элементы которой равны $1$ или $-1$.
\end{theorem}
\begin{proof}
Если мы рассмотрим координаты базиса $\Basis e$ относительно базиса $\Basis e$, то
\ShowEq{Minkowski basis 1}
Если вектор $\Vector e_k$ - времениподобный вектор, то,
согласно определениям
\ref{definition: Minkowski orthogonal basis},
\ref{definition: Minkowski orthonormal basis},
\def\TV{\text{- времениподобный вектор}}
\def\SV{\text{- времениподобный вектор}}
\ShowEq{Minkowski basis 2}
Из равенств \EqRef{Minkowski basis 2} следует\footnote{Очевидно,
что равенство \EqRef{Minkowski basis 2}
ничего не говорит о значении $g_{ij}(\Vector e_k)$,
если $i\ne k$, $j\ne k$, так как коэффициент при
$g_{ij}(\Vector e_k)$ в рассматриваемой сумме равен $0$.
Так как $g$ - симметричный тензор, то
\[
g_{kl}(\Vector e_k)=g_{lk}(\Vector e_k)\ \ \ k\le l
\]
При этом, если $k<l$, то $g_{kl}(\Vector e_k)=0$.
Однако, значение $g_{lk}(\Vector e_l)$ не определено.
}
\ShowEq{Minkowski basis 3}
Следовательно, $g_{kl}(\Vector e_k)$ произвольно, если $k>l$.
\end{proof}

Если в теореме
\ref{theorem: orthonormal basis in Minkowski space, positively defined Finsler metric}
ослабить требование и предположить произвольную финслерову метрику,
то мы встретим серьёзную проблему.
Множество векторов $\Vector e_{m+1}$,
удовлетворяющих системе линейных уравнений
\EqRef{choose em+1, Minkowski space},
порождает векторное пространство $\Vector V_{n-m}$ размерности $n-m$.
Если отношение ортогональности симметрично, то система линейных уравнений
\EqRef{choose em+1, Minkowski space}
эквивалентна системе линейных уравнений
\ShowEq{choose em+1 1, Minkowski space}
Из требования
\RefItem{metric tensor}
невырожденности финслеровой метрики и равенств
\EqRef{choose em+1 1, Minkowski space}
следует, что существует вектор
\ShowEq{v in Vn-m}
Утверждение
\EqRef{v in Vn-m}
гарантирует следующий шаг процедуры ортогонализации.
В случае произвольной финслеровой метрики,
мы не можем гарантировать, что процедура ортогонализации
может быть завершена при начальном выборе некоторого базиса $\Basis e'$,
так как очередной вектор оказался изотропным.

Задачи нахождения ортогонального базиса и приведения квадратичной формы
к сумме квадратов тесно связаны в геометрии евклидова пространства.
В пространстве Минковского, теорема
\ref{theorem: coordinates of metric tensor}
делает невозможной применимость алгоритма приведения квадратичной
формы к каноническому виду.

\section{Движение пространства Минковского}

Структура пространства Минковского близка структуре евклидова пространства.
Автоморфизм евклидова пространства называется движением.
Движение евклидова пространства является линейным преобразованием, отображающим
ортонормированный базис в ортонормированный.

Автоморфизм пространства Минковского так же называется движением.
Движение пространства Минковского является линейным преобразованием.
Если $\Basis e_1$, $\Basis e_2$ - ортонормированные базисы,
то существует единственное линейное преобразование, отображающее базис $\Basis e_1$
в базис $\Basis e_2$.
Однако из теоремы
\ref{theorem: motion Minkowski Space, 3d basis}
следует, что многообразие базисов пространства Минковского не замкнуто
относительно линейного преобразования.
Поэтому мы должны ослабить требования к определению движения пространства Минковского.

\begin{definition}
\label{definition: motion, Minkowski space}
Линейное преобразование пространства Минковского
отображающее по крайней мере один ортонормированный базис в
ортонормированный базис называется
\AddIndex{движением}{motion, Minkowski space}.
\qed
\end{definition}

Пусть движение $\Vector A$ пространства Минковского
отображает базис $\Basis e_1$ в базис $\Basis e_2$.
Пусть $e_i$ - матрица координат базиса $\Basis e_i$.
Тогда справедливо равенство
\ShowEq{motion, Minkowski space, matrix}

\begin{theorem}
\label{theorem: product of motions}
Пусть движение $\Vector A$ пространства Минковского
отображает ортонормированный базис $\Basis e_1$ в ортонормированный базис $\Basis e_2$.
Пусть движение $\Vector B$ пространства Минковского
отображает ортонормированный базис $\Basis e_2$ в ортонормированный базис $\Basis e_3$.
Тогда произведение движений $\Vector A\Vector B$ также является движением.
\end{theorem}
\begin{proof}
Поскольку произведение линейных преобразований является линейным преобразованием,
то утверждение теоремы следует из определения
\ref{definition: motion, Minkowski space}
и утверждения, что линейное преобразование $\Vector A\Vector B$
отображает ортонормированный базис $\Basis e_1$ в ортонормированный базис $\Basis e_3$.
\end{proof}

\begin{theorem}
\label{theorem: inverse motion}
Пусть линейное преобразование $\Vector A$ является движением.
Тогда линейное преобразование $\Vector A^{-1}$ является движением.
\end{theorem}
\begin{proof}
Пусть движение $\Vector A$ пространства Минковского
отображает ортонормированный базис $\Basis e_1$ в ортонормированный базис $\Basis e_2$.
Поскольку линейное преобразование $\Vector A^{-1}$
отображает ортонормированный базис $\Basis e_2$ в ортонормированный базис $\Basis e_1$,
то утверждение теоремы следует из определения
\ref{definition: motion, Minkowski space}.
\end{proof}

Согласно определению
\ref{definition: motion, Minkowski space},
множество движений $SO(\Vector V)$ пространства Минковского $\Vector V$
является подмножеством группы линейных преобразований $GL$.
Из теорем
\ref{theorem: product of motions},
ref{theorem: inverse motion}
следует, что на множестве движений $SO(\Vector V)$
определено ассоциативное произведение, которое имеет единицу
и обратный элемент.

Пусть движение $\Vector A$ пространства Минковского
отображает ортонормированный базис $\Basis e_1$ в ортонормированный базис $\Basis e_2$.
Пусть движение $\Vector B$ пространства Минковского
отображает ортонормированный базис $\Basis e_2$ в базис $\Basis e_3$.
Если базис $\Basis e_3$ не является ортонормированным,
то мы не знаем, является ли произведение $\Vector A\Vector B$ движением.
Следовательно, произведение движений не всегда определено и
множество движений $SO(\Vector V)$ пространства Минковского $\Vector V$
является не полной группой.

\begin{theorem}
\label{theorem: motion of Minkowski space}
Пусть координаты тензора $g$ определены относительно
ортонормированного базиса $\Basis e$.
Пусть движение пространства Минковского $\Vector V$
\DrawEq{motion of Minkowski space}{0}
отображает базис $\Basis e$
в ортонормированный базис $\Basis e'$.
Тогда\footnote{Поскольку при движении базис пространства не меняется, то отображения $g_{ij}$
также не меняются.}
\ShowEq{motion of Minkowski space 1}
\end{theorem}
\begin{proof}
Согласно определениям
\ref{definition: Minkowski orthogonal basis},
\ref{definition: Minkowski orthonormal basis},
векторы базиса $\Basis e$ удовлетворяют равенству
\DrawEq{Minkowski space, basis e}{motion}
и векторы базиса $\Basis e'$ удовлетворяют равенству
\DrawEq{Minkowski space, basis e'}{motion}
Из равенств
\eqRef{motion of Minkowski space}{0},
\eqRef{Minkowski space, basis e}{motion},
\eqRef{Minkowski space, basis e'}{motion}
следует
\ShowEq{motion of Minkowski space, bases e e'}
Так как $e^i_j=\delta^i_j$, то равенство
\EqRef{motion of Minkowski space 1}
следует из равенства
\EqRef{motion of Minkowski space, bases e e'}.
\end{proof}

\begin{corollary}
Пусть координаты тензора $g$ определены относительно
ортонормированного базиса $\Basis e$.
Пусть движение пространства Минковского $\Vector V$
\DrawEq{motion of Minkowski space}{}
отображает базис $\Basis e$
в ортонормированный базис $\Basis e'$.
Тогда
\ShowEq{motion of Minkowski space 2}
\qed
\end{corollary}

Теорема
\ref{theorem: motion of Minkowski space}
также следует из утверждения,
что координаты движения $\Vector A$ относительно базиса $\Basis e$
совпадают с координатами базиса $\Basis e'$
\ShowEq{motion of Minkowski space 3}

\begin{corollary}
\label{corollary: motion of Minkowski space}
Пусть
\ShowEq{orthonormal bases 1 2}
- ортонормированные базисы.
Пусть
\ShowEq{motion A basis 2 1}
координаты базиса $\Basis e_2$ относительно базиса $\Basis e_1$.
Тогда
\DrawEq{orthonormal bases of Minkowski space}{}
где
\ShowEq{motion of Minkowski space g 1}
координаты метрического тензора относительно базиса $\Basis e_1$.
\qed
\end{corollary}

\begin{theorem}
\label{theorem: Bases e e' motion, Minkowski space}
Пусть бесконечно малое движение
\DrawEq{Bases e e' A 1, Minkowski space}{}
отображает ортонормированный базис $\Basis e$
в ортонормированный базис $\Basis e'$
\ShowEq{Bases e e' motion, Minkowski space}
Тогда
\ShowEq{Bases e e' 3, Minkowski space}
\ShowEq{Bases e e' 5, Minkowski space}
\end{theorem}
\begin{proof}
Для $k\le l$ из равенств
\EqRef{Bases e e' motion, Minkowski space},
\EqRef{infinitesimal transformation of metric, Minkowski space},
следует
\ShowEq{Bases e e' 1, Minkowski space}
Из равенств
\eqRef{Minkowski space, basis e}{motion},
\eqRef{Minkowski space, basis e'}{motion},
\EqRef{Bases e e' 1, Minkowski space},
следует
\ShowEq{Bases e e' 3, Minkowski space}
\ShowEq{Bases e e' 2, Minkowski space}
Так как
\ShowEq{Bases e e' 4, Minkowski space}
то из равенства
\EqRef{Bases e e' 2, Minkowski space}
следует
\ShowEq{Bases e e' 3, Minkowski space}
\ShowEq{Bases e e' 6, Minkowski space}
Равенство
\EqRef{Bases e e' 5, Minkowski space}
следует
из равенств
\EqRef{metric is homogenious degree 0, 1},
\EqRef{Bases e e' 6, Minkowski space}.
\end{proof}

\begin{theorem}
\label{theorem: product of infinitesimal motions of Mincovsky space}
Произведение инфинитезимальных движений пространства Минковского
является инфинитезимальным движением пространства Минковского.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{product of infinitesimal motions, 1, Mincovsky space}
инфинитезимальные движения пространства Минковского.
Преобразование $fg$ имеет вид
\ShowEq{product of infinitesimal motions, 2, Mincovsky space}
Из теоремы
\ref{theorem: Bases e e' motion, Minkowski space},
следует, что координаты отображений $f$ и $g$ удовлетворяют равенствам
\ShowEq{product of infinitesimal motions, 3, Mincovsky space}
Из равенства
\EqRef{product of infinitesimal motions, 3, Mincovsky space}
следует
\ShowEq{Bases e e' 3, Minkowski space}
\ShowEq{product of infinitesimal motions, 4, Mincovsky space}
Следовательно, отображение $fg$ является
инфинитезимальным движением пространства Минковского.
\end{proof}

\begin{theorem}
\label{theorem: action real field, infinitesimal motion}
Пусть
\DrawEq{Bases e e' A 1, Minkowski space}{}
бесконечно малое движение.
Для любого $r\in R$, преобразование
\ShowEq{Bases e e' A 1r, Minkowski space}
является бесконечно малым движением.
\end{theorem}
\begin{proof}
Из равенства
\EqRef{Bases e e' 5, Minkowski space}
следует
\ShowEq{Bases e e' 3, Minkowski space}
\ShowEq{Bases e e' 5r, Minkowski space}
Утверждение теоремы следует из равенства
\EqRef{Bases e e' 5r, Minkowski space}
и теоремы
\ref{theorem: Bases e e' motion, Minkowski space}.
\end{proof}

\begin{theorem}
Множество инфинитезимальных движений является векторным пространством
над полем действительных чисел.
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: product of infinitesimal motions of Mincovsky space},
множество бесконечно малых движений порождает абелевую группу $g$.
Согласно теореме
\ref{theorem: action real field, infinitesimal motion},
определено представление поля действительных чисел в группе $g$.
Следовательно, группа $g$ является векторным пространством.
\end{proof}

%Чтобы увидеть структуру алгебры $g$, рассмотрим равенство
%\EqRef{Bases e e' 5, Minkowski space}.
%Следуя \citeBib{Rund Finsler geometry},
%рассмотрим матрицу

Так как отношение ортогональности не
симметрично, то это приводит к изменению структуры
метрического тензора в ортонормированном базисе.
В частности, так как скалярное произведение
\ShowEq{e k>l, Minkowski space}
не определено, то мы не можем требовать, что автоморфизм пространства Минковского
сохраняет скалярное произведение.

\begin{theorem}
Инфинитезимальное движение пространства Минковского
\DrawEq{Bases e e' A 1, Minkowski space}{1}
не сохраняет скалярное произведение.
Для заданных векторов $\Vector a$, $\Vector b$,
величину нарушения скалярного произведения можно
оценить выражением
\ShowEq{how much scalar product is not preserved}
\end{theorem}
\begin{proof}
Пусть инфинитезимальное движение пространства Минковского
отображает векторы $\Vector a$, $\Vector b$
в векторы
\ShowEq{Vectors a' b'}
\ShowEq{infinitesimal motion, Vectors a b}
Скалярное произведение векторов
\ShowEq{Vectors a' b'}
имеет вид
\ShowEq{infinitesimal motion, Vectors a b 1}
Равенство
\EqRef{how much scalar product is not preserved}
следует из равенства
\EqRef{infinitesimal motion, Vectors a b 1}.
\end{proof}

\section{Квазидвижение пространства Минковского}

Хотя структура множества $SO(\Vector V)$ движений
пространства Минковского $\Vector V$
не является полностью определённой группой,
множество $SO(\Vector V)$ является подмножеством группы $GL$
и действует однотранзитивно на многообразии базисов
пространства Минковского $\Vector V$.
Поэтому в множестве пассивных преобразований
векторного пространства $\Vector V$
мы можем выделить преобразования, сохраняющие структуру
пространства Минковского $\Vector V$.

\begin{definition}
\label{definition: quasimotion, Minkowski space}
Пассивное преобразование пространства Минковского
\DrawEq{transformation of basis, Minkowski space}{}
отображающее по крайней мере один ортонормированный базис в
ортонормированный базис называется
\AddIndex{квазидвижением пространства Минковского}{Quasimotion, Minkowski space}.
\qed
\end{definition}

Пусть квазидвижение $\Vector A$ пространства Минковского
отображает базис $\Basis e_1$ в базис $\Basis e_2$.
Пусть $e_i$ - матрица координат базиса $\Basis e_i$.
Тогда справедливо равенство
\ShowEq{quasimotion, Minkowski space, matrix}

Координаты вектора
\ShowEq{vector, Minkowski space}
преобразуются согласно правилу
\ShowEq{transformation of vector, Minkowski space}
Из равенств \EqRef{Euler theorem, Minkowski space, 8},
\EqRef{transformation of vector, Minkowski space}
следует
\ShowEq{transformation of metric, Minkowski space}
Из равенства \EqRef{transformation of metric, Minkowski space} следует
\ShowEq{transformation of metric, Minkowski space, 1}
Следовательно, $g_{ij}(\Vector a)$ является тензором.

\begin{remark}
До сих пор мы рассматривали метрику пространства Минковского $\Vector V$ как
набор функций $g_{ij}(\Vector v)$ вектора $\Vector v\in\Vector V$.
Поскольку базис $\Basis e$ задан, то мы имеем однозначное разложение
вектора $\Vector v$ относительно базиса $\Basis e$
\ShowEq{expansion vector v basis e}
Следовательно, мы можем рассматривать отображение $g_{ij}(\Vector v)$
как функцию $g_{ij}(v^1,...,v^n)$ переменных $v^1$, ..., $v^n$
\ShowEq{map gij v1 vn}
\qed
\end{remark}

\begin{theorem}
\label{theorem: quasimotion of Minkowski space}
Пусть координаты тензора $g$ определены относительно
ортонормированного базиса $\Basis e$.
Пусть квазидвижение пространства Минковского $\Vector V$
\DrawEq{transformation of basis, Minkowski space}{0}
отображает базис $\Basis e$
в ортонормированный базис $\Basis e'$.
Тогда
\ShowEq{quasimotion of Minkowski space 1}
\end{theorem}
\begin{proof}
Согласно определениям
\ref{definition: Minkowski orthogonal basis},
\ref{definition: Minkowski orthonormal basis},
векторы базиса $\Basis e$ удовлетворяют равенству
\DrawEq{Minkowski space, basis e}{quasimotion}
и векторы базиса $\Basis e'$ удовлетворяют равенству
\DrawEq{Minkowski space, basis e'}{quasimotion}
Из равенств
\eqRef{transformation of basis, Minkowski space}{0},
\eqRef{Minkowski space, basis e}{quasimotion},
\eqRef{Minkowski space, basis e'}{quasimotion}
следует
\ShowEq{quasimotion of Minkowski space, bases e e'}
Так как $e^i_j=\delta^i_j$, то равенство
\EqRef{quasimotion of Minkowski space 1}
следует из равенства
\EqRef{quasimotion of Minkowski space, bases e e'}.
\end{proof}

Из теорем
\ref{theorem: motion of Minkowski space},
\ref{theorem: quasimotion of Minkowski space}
следует, что множество
квазидвижений пространства Минковского
и множество
движений пространства Минковского
совпадают.

\begin{remark}

%\section{Геометрический объект в пространстве Минковского}

Множество квазидвижений порождает пассивное представление
не полной группы $SO(\Vector V)$.

Пусть $\Basis e_1$, $\Basis e_2$ - ортонормированные базисы
пространства Минковского $\Vector V$.
Согласно теореме
\ref{theorem: quasimotion of Minkowski space},
существует квазидвижение отображающее базис $\Basis e_1$
в базис $\Basis e_2$.
Поскольку не полная группа $SO(\Vector V)$ является подгруппой группы $GL$,
то это квазидвижение определено однозначно.
Следовательно, представление не полной группы $SO(\Vector V)$
на многообразии базисов пространства Минковского $\Vector V$
однотранзитивно.

%Так же как и в случае представления группы $GL$ в векторном
%пространстве, мы можем продлить представление не полной группы $SO(\Vector V)$
%на многообразие базисов (раздел
%\xRef{0701.238}{section: Basis Manifold for Vector Space}).

Поэтому определение геометрического объекта (раздел
\xRef{0701.238}{section: Geometric Object of Vector Space})
остаётся верным также в пространстве Минковского.
\qed
\end{remark}

\begin{theorem}
Пусть $\Vector A$ - квазидвижение, отображающее базис $\Basis e$
в базис $\Basis e'$
\ShowEq{quasimotion basis e e'}
Квазидвижение $\Vector A$ отображает отображение $g_{ij}(v^1,...,v^n)$
в отображение $g'_{ij}(v'^1,...,v'^n)$ согласно правилу
\ShowEq{quasimotion basis e e' g}
\end{theorem}
\begin{proof}
Из равенств
\EqRef{transformation of metric, Minkowski space, 1},
\EqRef{map gij v1 vn},
следует
\ShowEq{quasimotion basis e e' g 1}
Поскольку квазидвижение $\Vector A$ не изменяет вектор $\Vector v$, то
\ShowEq{quasimotion basis e e' g 2}
Из равенства
\EqRef{quasimotion basis e e' g 2}
следует
\ShowEq{quasimotion basis e e' g 3}
Равенство
\EqRef{quasimotion basis e e' g}
следует из равенств
\EqRef{quasimotion basis e e' g 1},
\EqRef{quasimotion basis e e' g 3}.
\end{proof}

\begin{theorem}
\label{theorem: Bases e e' quasimotion, Minkowski space}
Пусть бесконечно малое квазидвижение
\ShowEq{infinitesimal transformation of basis, Minkowski space}
отображает ортонормированный базис $\Basis e$
в ортонормированный базис $\Basis e'$
\ShowEq{Bases e e' quasimotion, Minkowski space}
Пусть координаты тензора $g$ определены относительно
ортонормированного базиса $\Basis e$.
Пусть координаты тензора $g'$ определены относительно
ортонормированного базиса $\Basis e'$.
Тогда
\ShowEq{Bases e e' 3, Minkowski space}
\ShowEq{infinitesimal transformation of metric, basis 4, Minkowski space}
\end{theorem}
\begin{proof}
Согласно
\EqRef{transformation of metric, Minkowski space, 1},
\EqRef{infinitesimal transformation of metric, Minkowski space},
следует, что метрический тензор испытывает бесконечно малое
преобразование\footnote{Мы используем равенство
\ShowEq{infinitesimal transformation of metric, basis 2, Minkowski space}
}
\ShowEq{infinitesimal transformation of metric, basis 1, Minkowski space}
Если $p=k$, то из равенства
\EqRef{infinitesimal transformation of metric, basis 1, Minkowski space}
следует
\ShowEq{infinitesimal transformation of metric, basis 1, p=k, Minkowski space}
При $k\le l$, согласно теореме
\ref{theorem: coordinates of metric tensor},
\ShowEq{infinitesimal transformation of metric, basis 3, Minkowski space}
Равенство
\EqRef{infinitesimal transformation of metric, basis 4, Minkowski space}
следует из равенств
\EqRef{metric is homogenious degree 0, 1},
\EqRef{infinitesimal transformation of metric, basis 1, p=k, Minkowski space},
\EqRef{infinitesimal transformation of metric, basis 3, Minkowski space}.
\end{proof}

Из теорем
\ref{theorem: Bases e e' motion, Minkowski space},
\ref{theorem: Bases e e' quasimotion, Minkowski space}
следует, что множество
бесконечно малых квазидвижений пространства Минковского
и множество
бесконечно малых движений пространства Минковского
совпадают.



==> Preface.MFinsler.Russian.tex <==
%auto-ignore
\input{Preface.MFinsler.Eq}

\chapter{Предисловие}

\section{Структура множества движений пространства Минковского}

Эта книга появилась в результате совместной работы авторов над
некоторыми вопросами, возникшими в результате анализа
статьи \citeBib{1107.5037}.
Евклидово пространство является предельным случаем пространства Минковского,
когда метрический тензор не зависит от направления.
Однако, хотя матрица метрического тензора относительно ортогонального
базиса евклидова пространства диагональна, аналог
\EqRef{coordinates of metric tensor, 1}
этой матрицы в пространстве Минковского является треугольной матрицей.
Это утверждение является крайне неудовлетворительным.

Поскольку теорема
\ref{theorem: coordinates of metric tensor}
не ограничивает значение элементов нижнего
треугольника матрицы
\EqRef{coordinates of metric tensor, 1},
то мы должны допустить, что это значение
произвольно. Это приводит к утверждению, что многообразие базисов
пространства Минковского больше чем многообразие базисов
евклидова пространства.
Когда мы завершили расчёты к секции
\ref{section: Example of Minkowski Space of Dimension 2},
мы поняли, что хотя рассматриваемое значение неизвестно, но не
произвольно.

Более существенной оказалась возможность упростить
уравнение %я
\xEqRef{1107.5037}{Bases e e' 5, Minkowski space}.
%\xEqRef{1107.5037}{infinitesimal transformation of metric, basis 4, Minkowski space}.
Уравнение
\EqRef{Bases e e' 5, Minkowski space}
напоминает аналогичное уравнение для евклидова пространства.
Из уравнения
\EqRef{motion of Minkowski space 1}
следует, что матрица движения пространства Минковского
близка к ортогональной матрице.

Поскольку множество $SO(\Vector V)$ движений пространства Минковского
размерности $n$ является подмножеством группы $GL(n)$ линейных преобразований,
то мы можем рассматривать произведение движений.
Однако множество $SO(\Vector V)$ не является замкнутым относительно
операции произведения.\footnote{Мы ожидаем статью, в которой покажем,
что в пространстве Минковского с нормой
\EqRef{example 3.2 of metric of Minkowski Space}
существуют движения, произведение которых не является движением.}
Другими словами, множество $SO(\Vector V)$
является не полной группой.\footnote{
Не полная группа является частным случаем не полной $\Omega$\Hyph алгебры.
\begin{definition}
Если операция $\omega\in\Omega$ определена не для всякого кортежа
элементов множества $A$,
то на множестве $A$ определена структура
\AddIndex{не полной $\Omega$\Hyph алгебры}{not complete Omega algebra}.
\qed
\end{definition}
Например, пусть на множестве $A$ определено
ассоциативное произведение, имеющее обратный элемент и единицу.
Таким образом, для любого $a\in A$ существует $b\in A$, для которых
определено произведение $ab$. Однако существуют $a$, $b\in A$, для
которых произведение неопределенно.
Тогда множестве $A$ называется
\AddIndex{не полной группой}{not complete group}.
}
Сейчас трудно сказать какие физические следствия может иметь это утверждение.
Однако так как не полная группа  $SO(\Vector V)$ имеет однотранзитивное
представление на многообразии базисов, и парное представление также однотранзитивно,
то мы можем рассмотреть определение геометрического объекта.

\section{Измерение угла}

В евклидовом пространстве существует два способа измерения угла.

Рассмотрим угол, образованный лучами $a$ и $b$,
которые имеют общую конечную точку называемую вершиной угла.
\ShowEq{angle a b}
Рассмотрим единичный круг с центром в вершине угла.
Мы можем определить величину угла как длину дуги, заключённой между
лучами $a$ и $b$.
Этот метод измерения угла используется в различных областях деятельности
человека, включая астрономию (раздел \citeBib{978-1898563020}-1.9).

Когда мы выполняем аналитические вычисления нам удобнее определять
косинус угла, опираясь на скалярное произведения векторов, параллельных
лучам $a$ и $b$.
Мы предполагаем, что измерения выполнены в псевдо евклидовом пространстве, где
скалярное произведение симметрично. Поэтому результаты рассмотренных методов
измерения совпадают.

Наблюдатель может выбрать произвольный метод измерения интервалов
длины и времени. Однако для того, чтобы один наблюдатель
мог сообщить результаты измерений другому наблюдателю, они
должны договориться об эталонах длины и времени.

Поэтому каждый наблюдатель выбирает свой базис таким образом,
что длина векторов базиса равна длине эталона.
Соответствующий базис мы будем называть нормальным.
Каждому базису сопутствует координатная система, построенная таким образом,
что координата $x^i$ точки на оси координат $X^i$ равна расстоянию от
начала координат.
В евклидовом или псевдоевклидовом
пространстве мы отождествляем каждую точку с радиус вектором этой точки.
Длина этого вектора является расстоянием от начала координат до рассматриваемой
точки. Квадрат длины этого вектора является квадратичной формой координат.
В случае евклидова пространства эта квадратичная форма положительно определена.

Наблюдатель может выбрать произвольный нормальный базис.
Соответственно, квадратичная форма, определяющая метрику, может иметь
произвольный вид.
Однако мы можем любую квадратичную форму привести
к каноническому виду (\citeBib{Kurosh: High Algebra},
с. 169 - 172).
Соответствующий базис является ортогональным базисом.
Ортогональный нормальный базис называется ортонормированным базисом.

Таким образом, для измерения пространственных и временных интервалов
наблюдатель пользуется ортонормированным базисом.\footnote{Этот шаг
в рассуждении кажется нелогичным.
Наблюдая свободное движение твёрдого тела и отвлекаясь от сил трения,
Галилей открывает закон инерции. Когда мы переходим от плоского
к искривленному пространству, естественно вместо движения по
прямой предположить движение по геодезической.
Но также как принцип Лагранжа, требование ортонормированности не
вытекает непосредственно из эксперимента.
Тем более кажется удивительным, что эксперимент подтверждает
эту точку зрения.}

В пространстве Минковского метрический тензор не является квадратичной
формой. Поэтому процедура экспериментального определения метрики
для заданного базиса является более сложной задачей.
Выполняя измерение расстояния в разных направлениях,
мы можем построить аналог единичной сферы в евклидовом пространстве,
а именно поверхность
\ShowEq{indicatrix}
которая называется индикатрисой.
В статье \citeBib{0009305},
Асанов рассмотрел, как опираясь на определённые физические гипотезы,
можно определить форму финслеровой метрики.

Согласно замечанию
\ref{remark: metric tensor depends on vector},
скалярное произведение в пространстве Минковского некоммутативно.
Поэтому косинус угла зависит от направления измерения.
Следовательно, в пространстве Минковского результаты рассмотренных выше методов
измерения не совпадают.
Соответственно, мы можем рассмотреть два различных определения ортонормированного базиса.

Согласно \citeBib{Rund Finsler geometry},
вектор $\Vector w$ ортогонален вектору $\Vector v$,
если вектор $\Vector w$ касателен гиперповерхности
\ShowEq{indicatrix 1}
гомотетичной индикатрисе.
Из равенства
\EqRef{Euler theorem, Minkowski space, 8}
следует, что вектор $\Vector w$, касательный гиперповерхности
\EqRef{indicatrix 1},
удовлетворяет уравнению
\ShowEq{indicatrix 2}
Из замечания
\ref{remark: metric tensor depends on vector}
следует, что вектор $\Vector w$ ортогонален вектору $\Vector v$,
если скалярное произведение
\ShowEq{indicatrix 3}
В этой статье мы рассматриваем определение
\ref{definition: Minkowski orthogonal basis}
ортогонального базиса, основанное на определении
\EqRef{indicatrix 2}
ортогональности.

Однако возможны и другие определения ортогональности,
например \citeBib{Asanov 2004,1112.5641}.
%Согласно \citeBib{Rund Finsler geometry},
%мы можем определить косинус угла, образованного
%векторами $\Vector v$, $\Vector w$, как выражение
%\ShowEq{Finsler cosine}

\section{Измерение скорости света}

Наблюдатель в общей теории относительности пользуется локальным
базисом в касательном пространстве, которое является пространством событий
специальной теории относительности.
Поэтому переход наблюдателя от одного локального базиса к другому
можно описать преобразованием Лоренца.

Когда геометрия пространства событий меняется настолько,
что преобразование базиса меняет свою структуру,
некоторые авторы воспринимают это изменение как нарушение
инвариантности Лоренца
(\citeBib{0711.0056}).
Если мы видим в эксперименте, что есть отклонение в структуре
преобразования Лоренца, то это является аргументом в пользу того,
что мы должны рассматривать новую геометрию.
Однако если новая геометрия верна, мы не должны ограничивать себя
инвариантностью Лоренца.
Наша задача - понять какую алгебру порождают преобразования новой
геометрии и как это влияет на принцип инвариантности.

Однако существует другая концепция нарушение
инвариантности Лоренца.
Эта концепция связана с зависимостью скорости света от направления
(\citeBib{1004.3007}, с. 7, \citeBib{1112.5641}, с. 12).
Эталоны длины и времени и скорость света неразрывно связаны
в теории относительности. Если мы знаем два из этих параметров,
мы можем определить третий.
Выбор геометрии также важен для определения зависимости
между рассматриваемыми параметрами.

Свет распространяется в финслеровом пространстве. Однако, так как
операция определения скорости - локальная операция, то
мы можем рассмотреть эту операцию в пространстве Минковского.
Мы полагаем, что вектор $\Vector e_0$ является времениподобным вектором,
а остальные векторы базиса являются пространственноподобными векторами.

Для того, чтобы измерять скорость света, мы должны предположить,
что нам заданы эталоны длины и времени.
Пусть финслерова метрика пространства событий имеет вид
(\citeBib{1004.3007}-(3))
\ShowEq{Speed of Light 1}
где $c$ - коэффициент, связывающий эталоны длины и времени,
и $F^2_3$ - положительно определённая финслерова метрика
3\Hyph мерного пространства.
Чтобы измерить скорость света в направлении в пространстве
\ShowEq{v1 v2 v3},
наблюдатель откладывает в заданном направлении
отрезок, длина которого равна эталону длины
\ShowEq{F=1}
и определяет время движения светового сигнала.
Поскольку вектор распространения света является изотропным,
то из равенства
\EqRef{Speed of Light 1}
следует
\ShowEq{Speed of Light 2}
Для любого выбранного направления в пространстве
\ShowEq{v1 v2 v3}
\ShowEq{Speed of Light 3}
Следовательно, время распространения света $v^0$ на заданное расстояние
не зависит от направления в пространстве.

Скорость света в рассматриваемой модели не зависит от направления
и равна $c$.
В пространстве Финслера финслерова метрика зависит от точки многообразия.
Поэтому процедура измерения скорости света должна быть выполнена
в бесконечно малой области.

\ifx\texFuture\Defined
Выражение для определения длины вектора $\Vector c$ имеет вид
\ShowEq{Speed of Light, 1}
$L_c$ - сумма положительных слагаемых,
которая выражает длину пути, пройденного световым сигналом.
$T_c$ - сумма отрицательных слагаемых,
которая выражает время, необходимое для путешествия светового сигнала.
Таким образом, скорость света в направлении
\ShowEq{c1 c2 c3}
имеет вид
\ShowEq{Speed of Light, 2}

У нас есть несколько замечаний по поводу равенства
\EqRef{Speed of Light, 2}.
\fi

Попытка понять, как взаимодействие элементарных частиц
и квантовых полей
может изменить геометрию пространства событий,
является одной из причин изучения финслеровой геометрии
(\citeBib{0009305,1004.3007}).
Без сомнения, только эксперимент может подтвердить,
является ли геометрия пространства событий финслеровой
и зависит ли скорость света от направления.\footnote{Физики проводят
эксперименты, проверяющие изотропность скорости света
(\citeBib{0305117,0706.2031,1008.1205}).
Задача экспериментов найти предел нарушения Лоренц инвариантности.

Даже
если окажется, что скорость света зависит от направления,
это не противоречит утверждению, что скорость света в заданном
направлении - это максимальная скорость передачи сигнала в
заданном направлении.
%Впрочем, топологические фокусы можно рассмотреть и в общей теории относительности.
}
Наша задача - найти эффективный инструмент для экспериментальной
проверки характера геометрии.

%В рассматриваемой задаче есть ещё одна возможность.
%Если финслерова метрика имеет вид
%\ShowEq{Speed of Light, 3}
%то мы можем также исследовать метрику вида
%\ShowEq{Speed of Light, 4}

